Responsive DNN Adaptation for Video Analytics against Environment Shift via Hierarchical Mobile-Cloud Collaborations

Mobile video analysis systems often encounter various deploying environments, where environment shifts present greater demands for responsiveness in adaptations of deployed "expert DNN models". Existing model adaptation frameworks primarily operate in a cloud-centric way, exhibiting degraded performance during adaptation and delayed reactions to environment shifts. Instead, this paper proposes MOCHA, a novel framework optimizing the responsiveness of continuous model adaptation through hierarchical collaborations between mobile and cloud resources. Specifically, MOCHA (1) reduces adaptation response delays by performing on-device model reuse and fast fine-tuning before requesting cloud model retrieval and end-to-end retraining; (2) accelerates history expert model retrieval by organizing them into a structured taxonomy utilizing domain semantics analyzed by a cloud foundation model as indices; (3) enables efficient local model reuse by maintaining onboard expert model caches for frequent scenes, which proactively prefetch model weights from the cloud model database. Extensive evaluations with real-world videos on three DNN tasks show MOCHA improves the model accuracy during adaptation by up to 6.8% while saving the response delay and retraining time by up to 35.5x and 3.0x respectively.

==> text/deprecated/01_intro.tex <==
\section{Introduction}\label{sec:intro}
Video analytics~\cite{wang2022pyramidfl,10.1145/3570361.3615749,295529,DBLP:conf/mobicom/ShiLJHHZYBX0YX24} with deep neural networks (DNN) have been extensively applied in Internet of Things (IoT) applications, including urban mobility~\cite{butler2020smart,mahrez2021smart,DBLP:conf/sensys/TangTHGS24}, enterprise surveillance~\cite{wang2017security,panchenko2018intelligent,10.1145/3384419.3430716,10.1145/3447993.3510590,10.1145/3636534.3649363}, traffic management~\cite{guidoni2020vehicular,10.1145/3447993.3448617}, and autonomous driving~\cite{yurtsever2020survey,10.1145/3495243.3560539,wang2018networking, 10.1145/3570361.3613280,10.1145/3560905.3568519}. 
Mobile video analytics perform DNN-based inference on mobile devices to deliver real-time responses~\cite{10.1145/3560905.3568546,bhardwaj2022ekya,khani2021real,10.1145/3625687.3625789,10.1145/3384419.3430721}.
Due to the resource constraints on mobile devices, dedicated \textit{expert models}, with compressed size and distilled knowledge from the large-scale \textit{teacher model}, are deployed to balance the prediction fidelity and processing throughput~\cite{molchanov2016pruning,gui2019model,295531,10.1145/3560905.3568520}.
These lightweight models memorize only limited video scenes and generalize poorly in scenes deviated from their training distributions (called \textit{domain shift}~\cite{lu2018learning,suprem13odin,wozniak2022deep}) and inevitably suffer from performance degradation~\cite{10.1145/3485730.3492886,10.1145/3666025.3699375,DBLP:conf/sensys/LuoHYWY024}. 

% To address this issue, continuous model adaptations that periodically detect domain shifts and accordingly update the expert model have gained recent popularity~\cite{luo2019taking,suprem13odin,zhou2022domain,khani2023recl,10.1145/3625687.3625804}.
% Two common strategies have been exploited:
% (1) \textit{Model retraining}~\cite{parisi2019continual,beaulieu2020learning,fang2024adashadow} updates the expert model parameters with freshly collected samples;
% (2) \textit{Model reuse}~\cite{khani2023recl} compares and selects one best candidate from a large zoo of history expert models to replace the obsolete one.
% Through adaptations, frameworks can sustain consistent performance despite frequent domain shifts.
To sustain stable DNN accuracy over time, continuous expert model adaptations need to be conducted upon detecting domain shifts~\cite{DBLP:conf/sensys/GaoTCC0H24,DBLP:conf/sensys/JiZ24,DBLP:conf/sensys/KaraKC00CWLA24,DBLP:conf/sensys/LiLL0024}, where two strategies are commonly exploited :
(1) \textit{Model retraining}~\cite{parisi2019continual,beaulieu2020learning,fang2024adashadow} updates the expert model parameters with freshly collected samples;
(2) \textit{Model reuse}~\cite{khani2023recl} compares and selects one best candidate from a history model zoo to replace the obsolete one.
However, due to resource-intensive computation or storage needs, existing solutions mostly host model adaptation services on the cloud~\cite{suprem13odin,khani2023recl,bhardwaj2022ekya}. This produces delayed responses to domain shifts:
First, as we show in Figure~\ref{fig:communication_overhead}, cloud-based model adaptation requires frequent data and model weight exchange (communication overhead time) between mobile and cloud~\cite{10.1145/3560905.3568538,10.1145/3485730.3485929,10.1145/3636534.3649359}, leading to considerable communication delays and bandwidth consumption;
Second, centralized adaptation paradigms make the cloud a single point of congestion, leading to poor scalability to the number of mobile devices with long cloud queuing delays.

This paper optimizes the \textit{response efficiency} of continuous model adaptation for mobile video analytics by efficiently exploiting mobile resources through a novel mobile-cloud collaborative paradigm.
The key intuition is to leverage lightweight mobile adaptation actions to reduce the frequency of requesting cloud adaptation services and avoid unnecessary mobile-cloud communications. 
Two technical challenges are thereby raised:
First, forcibly moving intact model reuse and retraining functions from cloud servers to mobile devices may induce excessive computation and storage load to onboard resources.
Second, considering the cloud network delays and mobile resource constraints, how to design a mobile-cloud collaboration algorithm taking advantage of both the low latency on the mobile and rich resources on the cloud stands out as another challenge.

% \textbf{Objective:} This paper seeks to optimize the response efficiency of continuous model adaptation for mobile video analytics by further leveraging limited mobile resources and designing an elaborated mobile-cloud collaboration paradigm.
% The key intuition is to reduce the frequency of requesting cloud adaptation services, avoid unnecessary mobile-cloud communications, and instead rely on mobile-hosted adaptation services as much as possible. 

% \textbf{Challenges:} Unleashing the power of mobile resources in continuous model adaptation can be technically challenging.
% First, the mobile resource constraints prohibit us from supporting computation-intensive model retraining executions or hosting a large zoo of history expert models in storage. 
% Forcibly transferring the intact model reuse or retraining service from the cloud to mobile devices can easily exceed their memory limits or produce even slower adaptation results.
% Second, when mobile devices can not completely replace cloud adaptation services, how to design appropriate mobile-cloud collaboration patterns, taking advantage of both the low latency on the mobile and rich resources on the cloud, stands out as another challenge.

We introduce \model, a mobile-cloud collaborative model adaptation framework for mobile video analytics. 
It distributes hierarchical adaptation functions between mobile and cloud resources.
We serve most model reuse and retraining requests locally on mobile through retrieval from a small expert model cache and updating the expert model with single-layer LoRA (Low-Rank Adaptation) fine-tuning while offloading intensive requests to the cloud server which hosts a full-fledged expert model database and runs end-to-end expert model retraining.
The cloud only works as a backup to the mobile when lightweight onboard services do not suffice to achieve the adaptation objective.

The design of \model includes three key components.
% First, \model organizes history expert models into a hierarchical semantic taxonomy shared between mobile and cloud. It provides a lightweight model indexing mechanism to quickly identify the suitable history expert model without model evaluation, which can run in real time on mobile devices. The domain semantics can be automatically discriminated from video frames by a multi-modal foundation model (FM) hosted on the cloud.
% Second, to circumvent model transmission delays, \model achieves onboard model reuse with a limited-size mobile model cache, which archives recently replaced and frequently accessed expert models. It also proactively prefetches expert models that may be reused soon from a cloud model database in the background. 
% Third, \model reduces the frequency of end-to-end retraining on the cloud by including a LoRA single-layer model fine-tuning on the mobile as an additional adaptation strategy, which only updates a small portion of parameters of a history expert model with minimum samples when it produces decent but suboptimal predictions in the new domain, instead of waiting to collect thousands of samples on the fly. 
First, \model offloads lightweight model adaptations to the mobile devices for better system responsiveness, which composes a two-tier adaptation hierarchy. It applies on-device model reuse and fast LoRA single-layer fine-tuning as immediate actions against domain shifts, before data transmission to the cloud for cloud model retrieval and end-to-end retraining.
Second, it constructs a structured model database organized by domain semantics, which can be analyzed by a foundation model (FM) on the cloud, to retrieve the fittest model candidate among history models in fast adaptations.
Third, \model maintains onboard model caches to store model weights for popular scenes, enabling seamless model switching with minimal onboard transmission delays. The mobile cache proactively interacts with the cloud model database for prefetching to ensure uninterrupted inference.


% First, \model organizes history expert models into a hierarchical taxonomy shared between mobile and cloud based on associated domain semantics, enabling efficient model retrieval for both reuse and retraining tasks. We deploy a multi-modal foundation model (FM) on the cloud to discriminate the domain semantics along predefined dimensions that could affect the expert model performance. The taxonomy provides a unique distance measure between different domains to measure the feasibility of cross-domain model reuse and retraining, which can run in real time on mobile devices. It enables a lightweight model indexing mechanism such that the suitable history expert model can be quickly identified without iteratively examining the model accuracy with a benchmark dataset~\cite{bhardwaj2022ekya,khani2023recl} or repeatedly updating a model selection network~\cite{khani2023recl,suprem13odin}.

% Second, \model achieves onboard model reuse without consulting the cloud and avoids model transmission delays through hosting a limited-size onboard expert model cache. 
% The model cache archives recently replaced and frequently accessed expert models for potential reuse in the future. 
% It also interacts with the cloud model database in the background to prefetch expert models that could be used shortly.

% Third, \model reduces the frequency of end-to-end model retraining on the cloud by including single-layer model fine-tuning on the mobile as an extra adaptation strategy. If the identified ``most suitable expert model'' produces decent but suboptimal predictions in the new domain, instead of initiating an end-to-end retraining task, we fine-tune a small portion of its parameters with minimal samples from the new domain, without waiting to collect thousands of samples on the fly. 
% Logically, fine-tuning bridges the gap between direct model reuse and end-to-end model retraining when an intermediate level of discrepancy exists between the new domain and its closest history domain.

We evaluate MOCHA with a large-scale real-world video dataset on three analytics tasks: object detection with YOLO~\cite{jocher2021ultralytics}, image classification with ResNet~\cite{he2016deep}, and semantic segmentation with Deeplabv3+~\cite{chen2018encoder}. We extensively compare it against state-of-the-art (SOTA) model adaptation systems.
The results show that \model supports more devices than SOTA methods in lower response delays with the same cloud resources. As the mobile device number scales, \model improves the accuracy during adaptation by up to 6.8\%, and saves the response delay and retraining time by $35.5\times$ and $3.0\times$. Ablation results validate that \model's superior performance mainly comes from the onboard adaptations of fine-tuning and reuse with mobile model cache.

In summary, the main contributions of this paper are:
\begin{itemize}[topsep=0pt,leftmargin=0.35cm]
    \item We propose a mobile-cloud collaborative continuous adaptation framework \model for effective mobile video analytics against runtime scene changes.
    \item We design an adaptation hierarchy of lightweight onboard model reuse, fine-tuning, and cloud retraining for better 
    responsiveness.
    \item We introduce an automated semantic model taxonomy for real-time domain metadata-based model retrieval used within adaptation strategies.
    \item We implement \model and perform extensive evaluations with a real-world video dataset, where \model saves the adaptation latency by up to $35.5\times$.
\end{itemize}

\begin{figure}[t!]
\includegraphics[width=0.95\linewidth]{figure/communication_overhead_in_reuse.pdf}
\caption{Communication overhead ratio comparison. The system first calculates the model to reuse and then transmits model weights to the mobile device. }
\label{fig:communication_overhead}
\end{figure}

% However, the mainstream video analytics tasks (\eg ResNet~\cite{he2016deep} for image classification~\cite{krizhevsky2017imagenet} and YOLO~\cite{jocher2021ultralytics} for object detection~\cite{zou2023object}) are very computation intensive, and their end-to-end retraining could cause an unaffordable workload to the limited onboard resources~\cite{khani2023recl}.
% For example, as we measured, an NVIDIA Jetson Nano platform is not able to run a YOLOV5-x model (218.8G FLOPs) and can only perform full retraining a YOLOv5-s model (17G FLOPs) at a speed of 1.72img/s with an image size of $640\times640$. 
% % \shengzhong{List the profiled results in a figure/table. Besides, claiming that YOLOV5-x can not run on Jetson Nano does not make sense.}
% Consequently, in mobile video analytics with limited compute resources and memory~\cite{weber2020emerging,10.1145/3447993.3483274,10.1145/3615587.3615990}, a series of small-scale models (called \textit{expert models})~\cite{kang2017noscope} that achieve comparable performance to a large-scale model in a single temporary scenario but lack generalizability into new scenarios, are trained on a cloud server and distributed to replace the large-scale accurate-yet-expensive model (called \textit{teacher model}) on devices~\cite{10.1145/3447993.3448628}, while reducing the resource overhead to an expert model.

% Due to the limited predictive capacity of expert models, the input data stream is discretized into segments, each representing a specific scenario. 
% We call such a scenario with a separate data distribution a ``domain'' and the change from one scenario to another a ``domain shift''.
% How to achieve timely detection of the domain shift phenomenon and accordingly arrange model adaptations to avoid long-time performance degradation becomes the core of designing a responsive mobile video analytics system. 
% Recent works in vision and system communities have proposed distinct solutions to tackling domain shift challenges. 
% For example, unsupervised clustering algorithms and lightweight gate networks are proposed to detect domain shifts~\cite{suprem13odin}. 
% Model reuse that applies historical models before a retraining task end is a temporary method to maintain the prediction quality against domain shifts~\cite{khani2023recl}. 
% GPU allocations are also widely studied to improve the performance in cases with multiple devices~\cite{bhardwaj2022ekya}.
% \shengzhong{The three examples are not very coherent. There is no conclusion on the limitation of existing works. Otherwise, we can move them to the related work section, or just remove them.}

% \textbf{Limitations.}  
% However, prior methods heavily depended on the cloud server for performing model adaptation computation but neglected the role that the mobile device can play. 
% The selection and scheduling of model adaptation tasks are all chosen to be decided on the server~\cite{}, leading to two fundamental limitations.
% % TRANSMISSION LIMITS RESPONSIVENESS
% First, cloud-based modal adaptation incurs inevitable network-related delays in multiple steps, \eg (1) between device-side data sampling and full uploads to the server and (2) between identification of the optimal model in the server and model distribution to the device for deployment. 
% Although the server possesses more compute resources, the communication overhead could wipe out the computational advantage. 
% Besides, the queueing delay before and after the cloud-side adaptation task occupies a non-negligible portion (Figure~\ref{fig:communication_overhead}), leading to long lags in adaptation.

% SERVER RETRAINING LIMITS SCALABILITY
% Second, massive retraining tasks on the server consume a majority of its computing resources. 
% Centralized retraining for many connected mobile devices could make the server a single point of efficiency bottleneck and failure.
% As shown in Figure~\ref{} \red{overall mAP on different numbers of devices}, the overall performance deteriorates as the number of devices rises.

% % FOR RESPONSIVENESS AND SCALABILITY, LAUNCH TWO CHANGES: TASK SCHEDULING, MODEL ADAPTATION
% \textbf{Our goal} in this paper is to build a scalable mobile video analytics system responding to environmental changes with shorter delays and achieving more stable performance addressing the aforementioned two fundamental limitations. 
% The key idea is to decentralize the model adaptation tasks to mobile devices to avoid server-side congestion and alleviate the impact of network transmission delays. 
% We allocate the model retraining workload between the device and the server by using a model selector with a model cache. 
% The mobile device is responsible for deciding when to start model adaptations and which model adaptation task should be launched, thereby reducing communication overhead and improving response time to domain shifts. 
% The logic behind our approach is that domain shifts generally exhibit temporal correlations. We can predict future scenes on the basis of this law, and pre-fetch the corresponding model from the cloud server to the model cache in advance so that we do not need to explicitly pause the model adaptations waiting for access to the server when a domain shift occurs. 
% % There have been works on the idea of temporal correlations of domains~\cite{khani2023recl}. However, they tend to use it to explain the value of storing historical information. 
% This paper is the first to use an on-device model cache to perform reusing on devices through this law to reduce the duration of performance degradation. 

% concrete challenges
% \textbf{Technical challenges.}
% Reusing models on devices necessitates selecting expert models that can be directly loaded, which leads to the creation of a model cache. Deploying these cache hierarchies involves addressing four key challenges.
% First, we should decide the time to change the current inference model with expert models in the model cache. For a single device, we cannot derive labels or determine the current domain without the help of the server. A responsive reuse demands us to detect data drifts without labels or domain information. 
% Second, we should design the strategy to select the optimal candidate when the cache hits or misses. Also due to a lack of labels and constraints on resources, we cannot follow the previous method of running a test epoch for the top-1 model. 
% Third, after the real-time reuse of expert models, we should determine how the server facilitates the replacement of expert models within the model cache. A static model cache is insufficient for maintaining a high hit rate to optimize system performance. Only a dynamic model cache that proactively pulls new expert models from the server during domain shifts can fully leverage responsiveness. 
% Fourth, we should launch appropriate retraining tasks to ensure that the cache can obtain sufficiently accurate expert models facing changing scenarios.

% \textbf{Contributions.} 
% To tackle these challenges above, we present our solution \model. It is the first end-to-end system that decentralizes model adaptation and task scheduling to devices for resource-efficient responsive video analytics, entailing three main ideas:
% \begin{enumerate}
%     \item  We design a model selection with cache hierarchies. A model taxonomy of all expert models is deployed on the server in the form of a prefix tree ordered by pre-selected domain attributes and shared by devices. A model selector with a model cache, which contains a fixed number of expert models transmitted from the model taxonomy, is deployed on each device. Our model selection design decentralizes task scheduling to devices and reduces the server overhead, enabling an efficient and scalable framework.
%     \item MOCHA designs a fast model adaptation procedure leveraging Foundation Models (FMs) and an Out-of-Distribution (OOD) algorithm. Our procedure can quickly select a suitable model from the cache without consulting the server and perform follow-ups when the cache misses, which can replace parts of traditional continuous learning. It is inspired by temporal correlations and has the best responsiveness among existing solutions. \shengzhong{Where does the spatial correlation come from?}
%     \item MOCHA designs resource allocations in model retraining to further improve the framework scalability and reduce the server overhead.
% \end{enumerate}






==> text/deprecated/02_motivation.tex <==
1
2
3
4
5
6
7
8
9
10
11
12
13
14
15
16
17
18
19
20
21
22
23
24
25
26
27
28
29
30
31
32
33
34
35
36
37
38
39
40
41
42
43
44
45
46
47
48
49
50
51
52
53
54
55
56
57
58
59
60
61
62
63
64
65
66
67
68
69
70
71
72
73
74
75
76
77
78
79
80
81
82
83
84
85
86
87
88
89
90
91
92
93
94
95
96
97
98
99
100
101
102
103
104
105
106
107
108
109
110
111
112
113
114
115
116
Responsive DNN Adaptation for Video Analytics against
Environment Shift via Hierarchical Mobile-Cloud Collaborations
Anonymous Author(s)
Abstract
Deploying small “expert DNN models” on mobile devices in place
of large-scale models and dynamically adapting them to evolving
runtime scenes proves promising for continuous mobile video an-
alytics. Existing model adaptation frameworks primarily operate
in a cloud-centric way, exhibiting degraded performance during
adaptation and delayed reactions to scene changes. Instead, this
paper proposes MOCHA, a novel framework optimizing the re-
sponsiveness of continuous model adaptation through hierarchical
collaborations between mobile and cloud resources. Specifically,
MOCHA (1) reduces adaptation response delays by performing on-
device model reuse and fast fine-tuning before requesting cloud
model retrieval and end-to-end retraining; (2) accelerates history
expert model retrieval by organizing them into a structured taxon-
omy utilizing domain semantics analyzed by a cloud foundation
model as indices; (3) enables efficient local model reuse by main-
taining onboard expert model caches for frequent scenes, which
proactively prefetch model weights from the cloud model database.
Extensive evaluations with real-world videos on three DNN tasks
show MOCHA improves the model accuracy during adaptation by
up to 6.8% while saving the response delay and retraining time by
up to 35.5× and 3.0× respectively.
1 Introduction
Video analytics [3, 68, 79, 81] with deep neural networks (DNN)
have been extensively applied in Internet of Things (IoT) appli-
cations, including urban mobility [7, 55, 75], enterprise surveil-
lance [19, 61, 78, 87, 93], traffic management [21, 76], and autonomous
driving [25, 26, 67, 77, 89]. Mobile video analytics perform DNN-
based inference on mobile devices to deliver real-time responses [2,
6, 36, 90, 94]. Due to the resource constraints on mobile devices,
dedicated expert models, with compressed size and distilled knowl-
edge from the large-scale teacher model, are deployed to balance
the prediction fidelity and processing throughput [20, 47, 57, 70].
These lightweight models memorize only limited video scenes and
generalize poorly in scenes deviated from their training distribu-
tions (called domain shift [49, 74, 82]) and inevitably suffer from
performance degradation [11, 46, 51].
In today’s mobile video analytics with deep neural networks
(DNN), numerous tasks are not confined to a single natural scene.
Instead, they are subject to various unpredictable environmental
variations (e.g., background or light condition changes), which al-
ter the data distribution of the collected video streams, posing sig-
nificant challenges to the quality of service (QoS). Although While
large-scale models exhibit robustness in dynamically changing en-
vironments (e.g., environment shifts), they cannot be directly ap-
plied to mobile video analytics, particularly on lightweight mobile
devices, where real-time inferences are performed to ensure re-
sponsiveness. Due to constraints in computational resources and
memory, only compressed expert models can be deployed on these
devices. However, such models can only memorize limited video
scenes and generalize poorly in environments that deviate from
their training distributions.
To alleviate performance degradation against environment shifts,
continuous expert model adaptations are conducted in previous
frameworks, where the cloud maintains a large-scale teacher model
and each mobile device deploys an expert model with distilled knowl-
edge from the teacher model. Two strategies are commonly ex-
ploited : (1) Model retraining [5, 17, 62] updates the expert model pa-
rameters with freshly collected samples; (2) Model reuse [35] com-
pares and selects one best candidate from a history model zoo to
replace the obsolete one. However, due to resource-intensive com-
putation or storage needs, existing solutions mostly host model
adaptation services on the cloud [6, 35, 74]. This produces delayed
responses to domain shifts: First, as we show in Figure 1, cloud-
based model adaptation requires frequent data and model weight
exchange (communication overhead time) between mobile and cloud [42,
52, 73], leading to considerable communication delays and band-
width consumption; Second, centralized adaptation paradigms make
the cloud a single point of congestion, leading to poor scalability
to the number of mobile devices with long cloud queuing delays.
This paper optimizes the response efficiency of continuous model
adaptation for mobile video analytics by efficiently exploiting mo-
bile resources through a novel mobile-cloud collaborative paradigm.
The key intuition is to leverage lightweight mobile adaptation ac-
tions to reduce the frequency of requesting cloud adaptation ser-
vices and avoid unnecessary mobile-cloud communications. Two
technical challenges are thereby raised: First, forcibly moving in-
tact model reuse and retraining functions from cloud servers to mo-
bile devices may induce excessive computation and storage load to
onboard resources. Second, considering the cloud network delays
and mobile resource constraints, how to design a mobile-cloud col-
laboration algorithm taking advantage of both the low latency on
the mobile and rich resources on the cloud stands out as another
challenge.
We introduce MOCHA, a mobile-cloud collaborative model adap-
tation framework for mobile video analytics. It distributes hierar-
chical adaptation functions between mobile and cloud resources.
We serve most model reuse and retraining requests locally on mo-
bile through retrieval from a small expert model cache and updat-
ing the expert model with single-layer LoRA (Low-Rank Adapta-
tion) fine-tuning while offloading intensive requests to the cloud
server which hosts a full-fledged expert model database and runs
end-to-end expert model retraining. The cloud only works as a
backup to the mobile when lightweight onboard services do not
suffice to achieve the adaptation objective.
The design of MOCHA includes three key components. First,
MOCHA offloads lightweight model adaptations to the mobile de-
vices for better system responsiveness, which composes a two-tier
adaptation hierarchy. It applies on-device model reuse and fast
LoRA single-layer fine-tuning as immediate actions against domain
1
117
118
119
120
121
122
123
124
125
126
127
128
129
130
131
132
133
134
135
136
137
138
139
140
141
142
143
144
145
146
147
148
149
150
151
152
153
154
155
156
157
158
159
160
161
162
163
164
165
166
167
168
169
170
171
172
173
174
Anon.
175
176
177
178
179
180
181
182
183
184
185
186
187
188
189
190
191
192
193
194
195
196
197
198
199
200
201
202
203
204
205
206
207
208
209
210
211
212
213
214
215
216
217
218
219
220
221
222
223
224
225
226
227
228
229
230
231
2321 5 10 20 50 75 100
Bandwidth (Mbps)
0
10
20
30
40
Response Time (s) 79.1%
65.5% 60.3%
43.1% 23.3% 16.8% 13.2%
Reuse Calculation Time
Communication Overhead Time
Figure 1: Communication overhead ratio comparison. The
system first calculates the model to reuse and then transmits
model weights to the mobile device.
shifts, before data transmission to the cloud for cloud model re-
trieval and end-to-end retraining. Second, it constructs a structured
model database organized by domain semantics, which can be an-
alyzed by a foundation model (FM) on the cloud, to retrieve the
fittest model candidate among history models in fast adaptations.
Third, MOCHA maintains onboard model caches to store model
weights for popular scenes, enabling seamless model switching
with minimal onboard transmission delays. The mobile cache proac-
tively interacts with the cloud model database for prefetching to
ensure uninterrupted inference.
We evaluate MOCHA with a large-scale real-world video dataset
on three analytics tasks: object detection with YOLO [32], image
classification with ResNet [24], and semantic segmentation with
Deeplabv3+ [10]. We extensively compare it against state-of-the-
art (SOTA) model adaptation systems. The results show that MOCHA
supports more devices than SOTA methods in lower response de-
lays with the same cloud resources. As the mobile device number
scales, MOCHA improves the accuracy during adaptation by up to
6.8%, and saves the response delay and retraining time by 35.5×
and 3.0×. Ablation results validate that MOCHA’s superior perfor-
mance mainly comes from the onboard adaptations of fine-tuning
and reuse with mobile model cache.
In summary, the main contributions of this paper are:
• We propose a mobile-cloud collaborative continuous adaptation
framework MOCHA for effective mobile video analytics against
runtime scene changes.
• We design an adaptation hierarchy of lightweight onboard model
reuse, fine-tuning, and cloud retraining for better responsive-
ness.
• We introduce an automated semantic model taxonomy for real-
time domain metadata-based model retrieval used within adap-
tation strategies.
• We implement MOCHA and perform extensive evaluations with
a real-world video dataset, where MOCHA saves the adaptation
latency by up to 35.5×.
2 Background and Motivations
Compared to the teacher model, expert models generalize poorly
against domain shifts. As Figure 2 shows, the accuracy degradation
of the teacher model remains within 15% across different domains,
while the expert model experiences up to a 52% accuracy drop.
Therefore, during frequent domain shifts, continuous adaptations
are needed to stabilize DNN accuracy. However, the two adapta-
tion strategies (i.e., reuse and retraining) face distinct challenges.
Reuse requires a trade-off between response speed and accuracy1 2 3 4 5 6
Domains
0.2
0.3
0.4
0.5
0.6
mAP
1 2 3 4 5 6
Domains
0
20
40
60
Change Ratio (%)
14.9%
52.3%
Teacher Model Expert Model
Figure 2: Teacher Model vs. Expert Model. The change ratio
denotes the ratio of accuracy drop in the current domain
over accuracy in the optimal domain, reflecting model gen-
eralizability in different environments.
Table 1: Resource metrics of different tasks. Bandwidth is 10
Mbps and model weight size is 14 MB.
Task Speed (FPS) Total Time (s) Memory (GB)
Inference 8.3 / 2.2
Onboard Fine-tune 9.7 120 2.6
Cloud Retrain 303 160 14.4
Onboard Reuse / 0.47 /
Cloud Reuse / 22.8 /
by making different choices of model selection within it while re-
training needs more compute resources and cannot provide a re-
sponsive solution at once [4]. To guarantee DNN accuracy, most
existing solutions [6, 35, 36, 74] completely offload these adapta-
tions to the remote cloud server, leading to suboptimal response
efficiency during domain shifts, due to mobile-cloud communica-
tion delays and cloud queuing delays [72]. To improve the respon-
siveness, our intuition is to deploy partial actions to mobile devices
and design a hierarchical adaptation system [44].
2.1 Hierarchical Model Adaptation
The “hierarchy” can be interpreted from two orthogonal per-
spectives: First, model adaptation tasks can be defined hierarchi-
cally: model reuse, fine-tuning a few layers, and end-to-end retrain-
ing, with increasing adaptability but decreasing efficiency. Second,
the model adaptation could happen collaboratively between mo-
bile devices and the cloud for balanced response efficiency and
adaptation effectiveness.
2.1.1 Mobile Fine-tuning vs. Cloud Retraining. The benefits
of model reuse in reducing model retraining have been highlighted
in RECL [35], while we further address the importance of light-
weight model fine-tuning that only selectively updates a few lay-
ers of a DNN. It is more computationally efficient than end-to-end
retraining and attains better adaptability than reuse when no suit-
able history expert model can be directly picked. As can be seen
from Table 1, although onboard fine-tuning takes longer per iter-
ation, its total update time is shorter due to the reduced training
iterations with fewer data and the absence of communication and
queuing delays encountered in cloud retraining tasks. Based on the
extent of domain shift, the combination of reuse, fine-tuning, and
retraining constitutes a more fine-grained action space for model
adaptation.
2.1.2 Mobile Reuse vs. Cloud Reuse. The limited mobile stor-
age and computation capacity have not been sufficiently explored
in model adaptations, where model reuse can demonstrate its value.
Intuitively, we make an analogy between mobile-vs-cloud resources
2
233
234
235
236
237
238
239
240
241
242
243
244
245
246
247
248
249
250
251
252
253
254
255
256
257
258
259
260
261
262
263
264
265
266
267
268
269
270
271
272
273
274
275
276
277
278
279
280
281
282
283
284
285
286
287
288
289
290
Responsive DNN Adaptation for Video Analytics against Environment Shift via Hierarchical Mobile-Cloud Collaborations
291
292
293
294
295
296
297
298
299
300
301
302
303
304
305
306
307
308
309
310
311
312
313
314
315
316
317
318
319
320
321
322
323
324
325
326
327
328
329
330
331
332
333
334
335
336
337
338
339
340
341
342
343
344
345
346
347
348
and the hierarchical storage of computer systems. We have limited
but fast-accessing resources (“cache”) on mobile devices, and abun-
dant but distant resources (“main memory”) on the cloud server.
From the storage aspect, saving a few frequent expert models on
the mobile can save remote access delays. From the computation as-
pect, distributing lightweight fine-tuning on mobile devices while
centralizing heavyweight retraining on the cloud can balance the
response efficiency and processing throughput in expert model up-
dates.
For example, in object detection tasks, a YOLOv5-s model (17M
FLOPs) weights file is about 14MB, thus we can store multiple
expert models on the mobile device. As shown in Table 1, if the
expert model is cached onboard, we can directly load it in 0.47s,
without waiting for the cloud dispatch, thus improving the overall
response speed [86]. We further analyze the scalability of mobile
device numbers between local reuse and cloud reuse. As Figure 3
shows, onboard retrieval exhibits magnitudes shorter response de-
lays than cloud model retrieval, which gap is further pronounced
when more mobile devices need to be served by the cloud. Intu-
itively, the temporal correlations presented in domain shifts make
onboard model caching a promising solution. For example, recur-
rent light condition changes when driving through consecutive
tunnels can iterate between scenes of daytime and night, thus lead-
ing to frequent switches between two expert models.
2.2 Semantic-Indexed Model Retrieval
One critical step to hierarchical adaptations is the efficient re-
trieval of the best candidate for the new domain from history ex-
pert models. Besides iterating over all models with a benchmark
dataset, recent studies have employed unsupervised clustering [74]
or maintained a gate network [35] for expert model selection. How-
ever, these learnable methods require frequent updates when the
model set changes. We argue that they all overlook recognizable
but critical semantic information of the deployed environments
(i.e., time, weather) [28], which can be used to organize history ex-
pert models into a structured database, instead of a disorganized
model zoo, to improve the model retrieval efficiency.
2.2.1 Domain Semantics Recognition. Some domain seman-
tics can be easily recognized by general foundation models (FM)
in a zero-shot way [9, 18, 71], which has been pre-trained on mas-
sive data and can be used for diverse downstream tasks. Existing
FMs, like LLaVA [48], have been pre-trained to comprehend multi-
modal input by connecting image input with a text prompt [50].
In Table 2, we use LLaVA to recognize the time, weather, and lo-
cation of an image with a dedicated prompt. It achieves promis-
ing accuracy in discriminating domains. The computation for a
640 × 640 image takes 500ms on an NVIDIA RTX4090 GPU. We
request human operators to provide a subset of domain semantic
dimensions with value options as a one-time effort to facilitate ex-
pert model management, while other uninterpretable factors are
implicitly handled in model continual learning.2 4 6 8 10
Device Number
0
20
40
60
Time (s)
22.8
29.2
36.8 41.2
49.4
0.47 0.47 0.47 0.47 0.47
Onboard Reuse Cloud Reuse
Figure 3: Onboard Reuse v.s. Cloud Reuse.0 1 2 3 4 5 6
Distance
70
80
90
100
Trend in mAP (%)
1 2 3 4 5 6
Domains
1.0
0.5
0.0
PCC
Domain 1 (STREET_OVERCAST_DAY)
Domain 2 (STREET_CLEAR_ALL-TIME)
Domain 3 (STREET_SNOWY_DAY)
Domain 4 (HIGHWAY_CLEAR_DAY)
Domain 5 (STREET_SNOWY_NIGHT)
Domain 6 (STREET_CLEAR_DAY)
Figure 4: Reuse on similar domains. Pearson correlation co-
efficient (PCC) is calculated from the distance and mAP for
each validation domain.
2.2.2 Domain Semantics Utilization. The semantic dimensions
1 can build a hierarchical taxonomy and a distance space on dif-
ferent domains, which can be directly used to retrieve the fittest
model candidate in fast adaptations. We hypothesize that the semantic-
level distance can work as an indicator of cross-domain model
reuse and retraining effectiveness. We conduct a few experiments
to analyze the cross-domain gaps for empirical validation. Intu-
itively, two domains are similar if they share most attributes but
differ in a few. If all attributes match, the domains are identical.
Direct Reuse: We use data from BDD100K [88] and a set of
YOLOv5-s pre-trained models to perform object detection on more
than 10 validation domains divided by three attributes “location”,
“weather”, “time_of_day”, and record the mean Average Precision
(mAP) as detection accuracy. We use a distance (introduced in §5.1
of MOCHA) as domain similarities. We list 6 domains of model per-
formances in Figure 4. More similar domains tend to have higher
cross-domain accuracy, and the highest accuracy is achieved in the
training domain (i.e., distance=0). The semantic similarity exhibits
a strong negative correlation with model performance, with the
overall average Pearson correlation coefficient (PCC) exceeding -
0.82. With more shared attributes, domain distributions become
closer or even overlapped. In the overlapped scenes, models from
both domains produce similar outputs and close accuracy.
Lightweight Fine-tuning: We also test whether models from
similar domains are more suitable for fast fine-tuning. We use the
same data and models to conduct a fine-tuning task with fixed
epochs while freezing all but a single layer of the model. In Figure 5,
we fine-tune models from all domains on the “STREET_CLEAR_DAY”
domain and test mAP on its validation data. The results show that
more similar domains can also obtain faster convergence and bet-
ter accuracy improvement after fine-tuning. Thus, semantic simi-
larity can also be used as an indicator for cross-domain fine-tuning.
3
349
350
351
352
353
354
355
356
357
358
359
360
361
362
363
364
365
366
367
368
369
370
371
372
373
374
375
376
377
378
379
380
381
382
383
384
385
386
387
388
389
390
391
392
393
394
395
396
397
398
399
400
401
402
403
404
405
406
Anon.
407
408
409
410
411
412
413
414
415
416
417
418
419
420
421
422
423
424
425
426
427
428
429
430
431
432
433
434
435
436
437
438
439
440
441
442
443
444
445
446
447
448
449
450
451
452
453
454
455
456
457
458
459
460
461
462
463
464
Table 2: Examples of foundation model (FM)-based domain semantic discrimination.
Prompt Identify the location, the weather, and the time in the image.
Respond in three words in the order of location, weather, and time, separated by commas, all lowercase.
Images
Responses street, rainy, night highway, snowy, daytime residential, clear, daytime0 10 20 30 40
Epochs
40
50
60
70
80
Epoch mAP(%) Dist=0
Dist=2
Dist=4
Dist=6
0 2 4 6
Distance
60
65
70
75
80
Fine-tuned mAP(%)
Figure 5: Fine-tuning on similar domains. Models from do-
mains at varying distances are used as starting points for
fine-tuning on the same dataset.
3 MOCHA Framework
3.1 Overall Architecture
As Figure 6 shows, MOCHA is a mobile-cloud collaborative model
adaptation framework for continuous mobile video analytics with
resilient prediction fidelity. Upon a domain shift, the system should
calibrate the mobile-deployed model to recover high accuracy within
a short response latency. We consider a cloud server with power-
ful compute and storage resources, and a set of distributed mobile
devices with constrained compute and communication resources
(e.g., NVIDIA Jetson Nano, TX2). MOCHA offloads low-latency
adaptation to mobile devices through lightweight computations
(i.e., local reuse and fast fine-tuning), with background support
from the cloud server through heavyweight computations (i.e., end-
to-end retraining).
Optimization Objective: The core tasks of continuous modal
adaptation include “detecting when the domain shift happens” and
“adapting the mobile-deployed expert model”, optimizing the respon-
siveness (i.e., finish adaptation in a short time) and scalability (i.e.,
support more mobile devices) of adaptations, under the constraints
of mobile resources and mobile-cloud network delays. MOCHA
performs domain shift detection on mobile devices, implements
model-cache-based reuse and LoRA single-layer fine-tuning as im-
mediate onboard reactions, and leaves accurate model retrieval from
a full-fledged model database and end-to-end retraining on the
cloud as backup strategies. MOCHA’s response efficiency bene-
fits from its mobile-cloud collaborative nature on reuse and update
strategies, as defined below.
• Model Reuse: If the exact or a similar domain has appeared
in the past, we directly retrieve and use the previously trained
model from the mobile model cache or the cloud model database
as a response.
1The selection of attributes’ dimensions is orthogonal to this paper, which is hard to
analyze quantitatively. We assume users provide parts of these parameters and the
system can construct the taxonomy offline using a few-shot validation dataset.Mobile
Devices
Raw Data
Cloud Model
Database
Mobile Model
Cache
Executor
Outputs Expert Model
Raw Data Data Labels Model
Request
Cloud
Data Pool
Mobile
Data Buffers
Annotator
Data
Annotator
Domain
Discriminator
Data Transmission Flow
Model Transmission Flow
Model
Dispatch
Domain
Shift Detector
Cloud
Server
Deployed
Expert Model
Semantical
Model Taxonomy
Semantical
Model Taxonomy
Historical
Domain Data
• Raw Data
• Labeled Data
Cloud Model Adaptation Retraining
Mobile Model
Adaptation
Fine-Tuning
Reuse
Figure 6: Architecture of MOCHA.
• Model Update: If no previous model can fit in the current do-
main, we update part or all of a model’s parameters through
lightweight onboard fine-tuning or end-to-end retraining on the
cloud server to respond with delays.
MOCHA’s performance highly relies on effective and efficient his-
tory model retrieval from past domains. MOCHA leverages meta-
level domain semantics identified by a multi-modal foundation model,
as indices to construct a domain taxonomy for real-time expert
model retrieval. Below, we list the main mobile and cloud compo-
nents in MOCHA.
3.1.1 Mobile Components. Besides regular model inference, the
mobile device periodically detects the occurrence of domain shifts
and performs fast onboard model reuse and fine-tuning, through
the following four modules.
• Executor: It performs inference on the real-time video stream.
Besides, a lightweight domain shift detector is integrated to de-
tect potential distributional drifts.
• Mobile Model Cache: It stores a few expert models that could
be reused shortly. At the meta-level, it keeps a copy of the se-
mantic model taxonomy (synchronized with the cloud server)
to assist in model selection.
• Mobile Data Buffer: Two data buffers are used to store the
real-time data stream awaiting inference and the labeled data
prepared for fine-tuning.
4
465
466
467
468
469
470
471
472
473
474
475
476
477
478
479
480
481
482
483
484
485
486
487
488
489
490
491
492
493
494
495
496
497
498
499
500
501
502
503
504
505
506
507
508
509
510
511
512
513
514
515
516
517
518
519
520
521
522
Responsive DNN Adaptation for Video Analytics against Environment Shift via Hierarchical Mobile-Cloud Collaborations
523
524
525
526
527
528
529
530
531
532
533
534
535
536
537
538
539
540
541
542
543
544
545
546
547
548
549
550
551
552
553
554
555
556
557
558
559
560
561
562
563
564
565
566
567
568
569
570
571
572
573
574
575
576
577
578
579
580Cloud Server
Annotator
Data Pool
Sensing
Stream Outputs
Mobile Device
Expert Model
Data Buffer
Raw Data Data Labels
Figure 7: Data transmission flow.
• Mobile Model Adaptation: Its frontend performs direct model
reuse or fine-tuning based on the mobile model cache. If needed,
its backend interacts with the cloud for retrieval from the cloud
model database or end-to-end retraining for ultimate adapta-
tion.
3.1.2 Cloud Components. The cloud server stores history mod-
els collected from its connected mobile devices and performs com-
putation tasks in the background to assist the mobile device com-
ponents, with the following four modules.
• Annotator: A large-scale teacher model is deployed to anno-
tate the mobile-uploaded samples and a multi-modal foundation
model is used to recognize the meta-level domain semantics (i.e.,
time, weather, location).
• Cloud Model Database: It stores expert models in historical
domains based on predefined semantic dimensions, enabling ef-
ficient model retrieval. A taxonomy updating algorithm is de-
signed along with retraining tasks.
• Cloud Data Pool: The labeled samples of historical domains
are stored for future domain retraining.
• Cloud Model Adaptation: It conducts end-to-end retraining
for new domains using data from the cloud data pool and dis-
patches the trained model to mobile devices.
3.2 Mobile-Cloud Collaboration Workflow
With the introduced mobile and cloud modules, we elaborate on
their collaboration procedure during adaptations. A standard data
transmission flow is shown in Figure 7. Although the frequency
of domain shifts is much lower than the sensor sampling rate (e.g.,
25 FPS), previous works [6, 35, 36] require continuous data upload-
ing for cloud-based domain shift detection. In contrast, MOCHA
avoids data transmission during periods without domain shifts by
hosting onboard domain shift detection.
This leads to two system states: during “regular inference time”,
only inference tasks and domain shift detection are conducted; dur-
ing “potential shift time”, continuous data uploading and annota-
tion are launched to confirm actual domain shifts and to prepare
data for adaptations. Following existing practices [6, 35], we set
fixed-length model-update windows (by default, 30 seconds) to en-
sure adequate time for fine-tuning data collection on mobile de-
vices and to provide a baseline for waiting times in specific system
states.
As a mobile-oriented framework, most MOCHA actions are trig-
gered and performed on the mobile, while the cloud passively serves
the submitted mobile requests. Within the collaboration, the mo-
bile activities include:
(1) It performs regular inference with the deployed expert model
on video frames and conducts domain shift detection based
on extracted sample features (§4.1). If distribution drifts are
detected, it enters potential shift time.
(2) In potential shift time, it uploads subsampled frames to the
cloud for (i) domain semantic discrimination for confirming
the domain shift, and (ii) sample annotations prepared for po-
tential adaptations. If the cloud confirms no domain shift hap-
pens, the false alarm is resolved and the mobile quits potential
shift time. Otherwise, the below adaptation actions are per-
formed.
(a) It immediately performs model reuse from the most simi-
lar domain(s) to recover accuracy (§4.2) and evaluates the
reused model with cloud-annotated samples. If an accu-
racy threshold is missed, a LoRA fine-tuning task starts
accordingly (§4.3).
(b) After step (a), if the new domain has not appeared in the
model taxonomy (i.e., an unseen domain), its end-to-end
training is needed. The mobile continuously uploads sam-
ples to the cloud while using the expert model from step
(a) for inference. Once enough data is aggregated, the new
model is trained and dispatched from the cloud to finish
the adaptation.
(c) After the adaptation sequence, the mobile quits potential
shift time and performs model replacement (§4.4) in the
background for the mobile model cache.
To assist the mobile adaptations, the cloud activities in each time
window include:
(1) Upon receiving mobile-uploaded samples, it uses the teacher
model to annotate task labels and uses the FM to discrimi-
nate domain semantics with dedicated prompts. It sends the
domain semantics back and stores the annotated samples in
its domain buffer.
(2) It serves model retrieval requests from mobile devices by dis-
patching the expert model to them.
(3) When one window ends, it updates the sample count of each
domain and launches end-to-end retraining if enough data is
accumulated.
(4) If an end-to-end retraining is finished, the new expert model
is stored in its model DB and indexed with domain semantics.
The model taxonomy (§5.1) is accordingly updated and syn-
chronized with all mobile devices.
4 Mobile Model Adaptation
This section answers four questions related to mobile adaptation
components: (1) how to detect domain shift? (2) how to load the op-
timal reuse model? (3) how to arrange onboard fine-tuning tasks?
(4) how to update the cache for future adaptations? An overview
of the mobile adaptation components is summarized in Figure 8.
4.1 Domain Shift Detection
The end-to-end domain shift detection is achieved through a
two-step process. First, we perform onboard domain shift detec-
tion to avoid unnecessary mobile-cloud data transmission during
regular inference time. Specifically, MOCHA applies a lightweight
out-of-distribution (OOD) approach [41] to determine the likeli-
hood of a domain shift without overconfidence bias. If an alarm is
fired, we switch from regular inference time to potential shift time.
Second, in potential shift time, the mobile device regularly uploads
5
581
582
583
584
585
586
587
588
589
590
591
592
593
594
595
596
597
598
599
600
601
602
603
604
605
606
607
608
609
610
611
612
613
614
615
616
617
618
619
620
621
622
623
624
625
626
627
628
629
630
631
632
633
634
635
636
637
638
Anon.
639
640
641
642
643
644
645
646
647
648
649
650
651
652
653
654
655
656
657
658
659
660
661
662
663
664
665
666
667
668
669
670
671
672
673
674
675
676
677
678
679
680
681
682
683
684
685
686
687
688
689
690
691
692
693
694
695
696Sensing Stream
Server
Inference OOD
Detection
ResultsRaw
Data
Optimal
Model
Inference
Model
OOD
Trigger
Fine-tuning
Fine-tuned Model
Executor
Reuse Model
Domain
Semantics
Reuse
Semantical
Taxonomy
Accuracy
Test
Replacement
Device
Model
Cache
Mobile
Adaptation
Figure 8: Responsive model adaptation design.
samples to the cloud to analyze the domain semantics to confirm
the actual domain shift. If the domain shift happens, mobile model
adaptation strategies are triggered.
We use a multi-dimensional Gaussian distribution to regress the
training distribution. Upon a model training finishes, we choose
features from a fixed layer, perform dimensionality reduction with
pooling, and record the mean ˆ���� and variance ˆΣ of the training fea-
tures. At runtime detection, the OOD score of a sample is calcu-
lated by feeding the extracted sample feature ���� into the equation
to get �� (���� ). The domain shift indicator of a window �������� (��) is
based on the aggregated sample OOD scores, as shown below.
ˆ���� = 1
����
∑
��:���� =��
�� (���� ), ˆΣ = 1
��
∑
��
∑
��:���� =��
�� (���� − ˆ���� ) (�� (���� − ˆ���� ) )�� ,
�� (���� ) = max
�� [− (�� (���� ) − ˆ���� )�� ˆΣ−1 (�� (���� ) − ˆ���� ) ],
�������� (�� ) = 1
��������
∑
0≤��<��������
�� (���� ),
where ���� is the sample count of class ��, �� is the training sample
count, and �������� is the sample count in a window.
We use the OOD score of point “�������� +�� ×������” as the threshold
of domain shift detection, with �� as a hyper-parameter. In §7.3 we
select a �� value that is relatively sensitive to distributional drift, to
ensure a high recall on the domain shift. The false positive alarms
fired by the mobile domain shift detector could be resolved by the
cloud domain discriminator (i.e., FM), without initiating meaning-
less adaptations. If the cloud FM indicates no domain shift, we exit
the potential shift time. Such collaborative domain shift detection
well balances the domain shift detection efficiency and quality.
4.2 Mobile Model Reuse
Once a domain shift is confirmed on the cloud, MOCHA per-
forms efficient model reuse as the immediate reaction. Technically,
the fitness of a history expert model should be defined by its accu-
racy in the new domain. However, annotating samples for the new
domain on the cloud and iterating over all history expert models
can be time-consuming, we instead use the semantical proximity
between domains as an efficient proxy of the model fitness, which
is calculated by a distance measure defined on the domain semanti-
cal features recognized by the cloud foundation model (as detailed
in §5.1). Since the semantical model taxonomy is synchronized on
each mobile device, model lookup can be performed locally on each
mobile device.
We first identify a “global optimal model” on the cloud model
database that is expected to achieve the best reuse accuracy. If it is
stored in the mobile model cache (i.e., cache hit), we directly load
it for reuse; otherwise if the “global optimal model” is not cached
onboard (i.e., cache miss), the reuse finishes in two steps. We iden-
tify another “local optimal model” from the mobile model cache
for temporary reuse before the “global optimal model” is down-
loaded from the cloud model database. In cache hit cases, MOCHA
eliminates the time of transmitting data and waiting for the cloud
to identify the optimal model. Otherwise, it involves cloud-based
model dispatch but still saves cloud queueing delays for domain
shift detection. Overall, the mobile model cache and onboard do-
main shift detector optimize the responsiveness of MOCHA’s model
reuse.
4.3 Mobile Model Fine-Tuning
Model reuse, although being most responsive, may lead to sub-
optimal adaptation quality in some cases. Thus, we further test the
reused expert model with a subset of labeled samples annotated by
the cloud. If the accuracy misses a threshold (by default 35% mAP
in object detection), at the end of one window, we launch an on-
board LoRA fine-tuning task with accumulated labeled samples in
the background, without interrupting the inference task.
Even though mobile fine-tuning takes longer for each iteration
than cloud retraining, it achieves completion faster overall as up-
dating single-layer parameters requires magnitudes fewer train-
ing samples. Moreover, fine-tuning avoids cloud queueing delays,
while retraining time could increase multiplicatively as more mo-
bile devices are connected to the cloud server. In our ablation stud-
ies (§7.4), fine-tuning is shown to be one critical factor in optimiz-
ing the accuracy during the adaptation. Notably, MOCHA does not
upload fine-tuned models to the cloud as it exhibits limited gener-
alizability into other mobile devices.
4.4 Mobile Model Cache Replacement
Similar to how the CPU cache prefetches memory pages after
a load, we proactively replace expert models in the mobile model
cache after reuse to ensure a higher likelihood of cache hits in the
next domain shift. Although future domain shift patterns can be
difficult to predict, we choose simple intuitions in cache replace-
ment.
First, the recurrence of domain shift indicates locality in model
reuse. For instance, in real-world driving, phenomena such as en-
tering and exiting tunnels or merging onto and off highways are
commonly observed. This indicates a pattern of frequent iteration
between two domains. Thus, we store the unloaded expert model in
the cache for potential use in the next fetch. Second, within a con-
tinuous video stream, the domain can not shift abruptly to seman-
tically distant domains. Instead, similar domains are more likely
to happen in the future. Therefore, we prefetch the expert model
for the most similar domain to the current domain with the most
shared attributes (e.g., from “daytime_clear_city-street)” to “day-
time_clear_highway” or “daytime_rainy_city-street”). The cache
replacement happens in the background through a best-effort man-
ner without strict deadlines or interrupting the inference task.
6
697
698
699
700
701
702
703
704
705
706
707
708
709
710
711
712
713
714
715
716
717
718
719
720
721
722
723
724
725
726
727
728
729
730
731
732
733
734
735
736
737
738
739
740
741
742
743
744
745
746
747
748
749
750
751
752
753
754
Responsive DNN Adaptation for Video Analytics against Environment Shift via Hierarchical Mobile-Cloud Collaborations
755
756
757
758
759
760
761
762
763
764
765
766
767
768
769
770
771
772
773
774
775
776
777
778
779
780
781
782
783
784
785
786
787
788
789
790
791
792
793
794
795
796
797
798
799
800
801
802
803
804
805
806
807
808
809
810
811
812
5 Cloud Model Adaptation
In addition to performing data annotations and domain discrim-
ination upon receiving uploaded samples from mobile, and man-
aging model dispatch in model reuse, the cloud is responsible for
maintaining a model taxonomy and serving end-to-end retraining
requests.
5.1 Semantic Model Taxonomy
Meta-level domain semantics are used as indices to perform ef-
ficient model retrieval and estimate the fitness of cross-domain ex-
pert model reuse. Our intuition is to organize extensive history
expert models into a hierarchical taxonomy rather than a disorga-
nized zoo, such that semantical comparison can be used to replace
repetitive model evaluations during selection. Below we introduce
how the domain semantics are organized and utilized.
We request the human operator to specify only the dimensions
of semantic attributes in advance (e.g., time, weather, and loca-
tion) while leaving their values open2. Based on these dimensions,
MOCHA generates the domain semantic taxonomy as a tree as vi-
sualized in Figure 9, where each layer corresponds to an attribute.
The child node is more concrete in domain semantics compared to
its parent node. The leaf nodes specify values in all attributes and
represent most fine-grained domains, while domains at non-leaf
nodes cover all their child domains. Each node on the semantic
model tree has an expert model in the cloud model DB and related
labeled data in the cloud data pool. Besides, we use a meta-level
taxonomy table to record the semantical model tree. It is synchro-
nized between the cloud and all mobile devices for model retrieval.
A semantic distance function �������� is defined to measure the
similarity of two domains as an indicator of cross-domain expert
model reuse accuracy. It also assists the expert model prefetch in
the mobile model cache management. The domain semantical dis-
tance is defined below.
�������� (��, ��) =
{
|���������� (��) − ���������� (��)|, �� ∈ ���� ∨ �� ∈ ����
�������� (��, ��) + �������� (��, ��), �� ∉ ���� ∧ �� ∉ ����
where �� and �� are the nodes of the tree, ���� means the subtree
of A, �� is the lowest common ancestor node of �� and ��. We em-
pirically show its effectiveness in proxying the cross-domain per-
formance in §7.3. Its computation is lightweight (Figure 10 as an
example) compared to the deep neural network (DNN) based gate
networks for expert model selection [35]. Meanwhile, with a new
domain, the taxonomy table can be easily extended without time-
consuming learning. Once enough samples are accumulated for a
new domain, its model can be end-to-end trained and archived on
the cloud. We add this new domain to the model taxonomy and
synchronize the new taxonomy to all mobile devices.
5.2 Cloud Model Retraining
In most situations, it is impossible to prepare training data for
all domains during the offline training, so we only train models for
a subset of domains as the initial point. At runtime, as we aggre-
gate enough data for a new domain, we initiate end-to-end training
2The foundation model (FM) possesses the capability of recognizing their values along
the given dimensions. Note the semantic dimensions are sorted in the decreasing order
of their impact on the model performance, which could be profiled offline with a
limited set of scenes.Attribute3
V1A1V1A2
V1A3
V1A1V1A2
V2A3
V2A1V2A2
V1A3
……
ROOT
Value3A1Value2A1Value1A1
Attribute1
Attribute2
V1A1V1A2 V1A1V2A2 V2A1V1A2 V2A1V2A2 V2A1V2A2 ……
Domain 1 Domain 2
Storage
Domains
Data
Model
Domains
Data
Model
Domains
Data
Model
Domain k
Semantic Model Tree
Domain
Data
Model
……
…… ……
……
……
……
Figure 9: Semantic model taxonomy on the cloud.Dist(A,B1)=2 Dist(A,B2)=3
C2
B1
B2
A
Figure 10: Distance algorithm examples.Currently Active Domains Taxonomy Domains
High-Level
Queue
Mid-Level
Queue
Low-Level
Queue
Figure 11: Multi-level queue.
and dynamically expand the model taxonomy. Meanwhile, an ex-
isting domain may meet with plenty of new data shifting from the
original data distribution. Although fast fine-tuning can partially
resolve the in-domain shift in some cases, it raises the necessity of
end-to-end retraining in other cases with significant shift3.
We store samples annotated by the teacher model and domain
semantics recognized by the FM for new domains and existing do-
mains currently under distribution drift. For storage efficiency, we
set an upper limit on the sample count per domain (by default,
1000). A non-leaf node in the taxonomy consolidates multiple sub-
domains, whose (re)training only begins when the node has data
from at least two subdomains or a new subdomain has appeared.
Moreover, the data for the non-leaf domain is sampled in a bal-
anced manner between subdomains for better generalizability.
5.3 Retraining Task Scheduling.
With the number of mobile devices rising, the cloud faces many
training tasks to run at a time and each task corresponds to a do-
main with a set of labeled frames. We treat this as a single-processor,
non-preemptive scheduling problem [53, 95] and apply a multi-
level queue scheduling algorithm on the cloud, as shown in Fig-
ure 11. Different queues are scheduled with priority scheduling,
where retraining tasks in lower-level queues only start when higher-
level queues are empty.
Three levels of queues are maintained, and different scheduling
policies are applied within each level of task queues. At the end of
each window, two meta-information—the currently active domain
3This is regarded as distributional drift caused by unexplainable factors where conven-
tional continuous learning algorithms can fit in to tackle the catastrophic forgetting
problem, which is beyond the scope of this paper.
7
813
814
815
816
817
818
819
820
821
822
823
824
825
826
827
828
829
830
831
832
833
834
835
836
837
838
839
840
841
842
843
844
845
846
847
848
849
850
851
852
853
854
855
856
857
858
859
860
861
862
863
864
865
866
867
868
869
870
Anon.
871
872
873
874
875
876
877
878
879
880
881
882
883
884
885
886
887
888
889
890
891
892
893
894
895
896
897
898
899
900
901
902
903
904
905
906
907
908
909
910
911
912
913
914
915
916
917
918
919
920
921
922
923
924
925
926
927
928
and model accuracy in the last window—are uploaded for each re-
training task from mobile devices to determine the corresponding
queues they belong to.
• High-level queue: Training tasks of currently active domains
that have not appeared in the model taxonomy, where an expert
model from a similar domain is temporally reused but with sub-
optimal accuracy. Its tasks are scheduled with a First-In-First-
Out (FIFO) policy.
• Mid-level queue: Retraining tasks of currently active domains
that are already in the taxonomy. Its tasks are scheduled in the
increasing order of accuracy in the last window.
• Low-level queue: Retraining tasks of domains in the model
taxonomy but not currently active, scheduled with FIFO policy.
Non-leaf nodes are in the low-level queue because they are only
used for temporary reuse.
6 Implementation
We implemented MOCHA with 5.8K lines of Python code and
implemented all neural networks under PyTorch [63]. The hard-
ware and software setups are specified below.
Hardware Configurations. As shown in Figure 12, we use a
workstation equipped with an Intel Xeon Gold 5420+ CPU, 128
GB memory, and an NVIDIA RTX 4090 GPU (24 GB RAM) as the
cloud server. For mobile devices, we use multiple NVIDIA Jetson
TX2 and Jetson Nano boards, all configured to MAXN mode to en-
sure stable performance. Each mobile device runs MOCHA’s com-
ponents alongside a separate input thread to simulate the video
stream.
Software Implementation. We use wondershaper [16] to sim-
ulate different network conditions (by default, 10Mbps). We use
llava-v1.6-vicuna-7b as our FM to discriminate domain semantics.
The network data transmission is implemented via TCP Socket
APIs. We launch a socket server on the cloud with a fixed port. Each
mobile device connects to the port and is allocated an ID stored on
the cloud. When transmitting data, the socket API automatically
adds its ID to the TCP packages and the cloud can correctly pro-
cess data from different devices. For retrieval requests, a temporary
socket connection is established to transmit model weights with-
out an allocated ID. On the mobile side, model inference, model
adaptation, and data transmission are executed in separate threads,
and the model cache has 3 slots. On the cloud server, data anno-
tation, socket connections, and database updates are managed as
distinct threads.
7 Experiments
In this section, we report the evaluation results of MOCHA on
two video-analytics tasks. We first present the methodology (§7.1)
and end-to-end results (§7.2), then show micro-performance anal-
ysis (§7.3), ablation studies (§7.4) and mobile overhead (§7.5).
7.1 Methodology & Setup
7.1.1 Dataset. We evaluate MOCHA under 3 randomly gener-
ated domain sequences in BDD dataset [88]. This dataset consists
of 100K 1280 × 720 colored videos collected with dashboard cam-
eras from diverse environments. Ten object classes, along with 108
domains and 3 semantic attributes, are included. In each domain
sequence, we concatenate one video with another video from the
Figure 12: Cloud server and mobile devices.
same domain when a video ends and change the domain after a
fixed number of videos like past frameworks [35, 74]. By contin-
ually changing domains, we simulate different domain shifts and
evaluate MOCHA’s performance. For image classification, we cre-
ate the dataset by cropping images from the BDD dataset, using
YOLO model annotations to obtain the desired size (1.4× to the
bounding box size) of images with both the domain background
and target objects.
7.1.2 Models. We leverage YOLOv5-5.0 implementation for ob-
ject detection, with YOLOv5-s and YOLOv5-x as expert and teacher
models respectively. 4 For image classification, we use ResNet im-
plementation in torchvision [13], with ResNet18 and ResNet152 as
expert and teacher models respectively. For semantic segmenta-
tion, we use DeepLabv3+MobileNet and DeepLabv3+ResNet101 as
expert and teacher models respectively. We pre-train expert mod-
els of 12 random domains and store them in the model database
according to configurations to simulate the real-time adaptations.
7.1.3 Metrics. To evaluate the system accuracy during continu-
ous adaptation, we compare the mobile inference results with la-
bels annotated by the more accurate and more expensive teacher
model and ground-truth labels manually annotated from BDD. Specif-
ically, we use mean Average Precision (mAP) for object detection
tasks, classification accuracy (ACC.) for image classification tasks
and Mean Intersection over Union (MIoU) for semantic segmenta-
tion tasks. In end-to-end evaluations, the following metrics are
compared:
• Recovery accuracy: Since most windows do not experience do-
main shifts, the overall model accuracy may not appropriately
reflect the adaptation performance. Instead, we only measure
the model accuracy during the recovery period from detecting
domain shifts to the completion of adaptation. For a fair com-
parison, we regard the time when the slowest framework, RECL,
deploys a new model as the end of recovery, such that all com-
pared frameworks share the same recovery period.
• Response delay: It is defined as the duration from when do-
main shifts are detected to when the first model adaptation ac-
tion is performed.
• Retraining time: It is defined as the duration from starting an
end-to-end retraining on the cloud to deploying the retrained
model on the device.
7.1.4 Baselines. The compared baselines include:
• No Adaptation: Pre-trained models are deployed on edge de-
vices without any adaptation.
• ODIN: It detects and recovers from data drifts based on the sim-
ilarity of video data and an autoencoder-based model selection.
4The version of Python pre-installed on Nvidia Jetson TX2 is 3.6.9, and higher versions
of YOLO are not supported in this environment.
8
929
930
931
932
933
934
935
936
937
938
939
940
941
942
943
944
945
946
947
948
949
950
951
952
953
954
955
956
957
958
959
960
961
962
963
964
965
966
967
968
969
970
971
972
973
974
975
976
977
978
979
980
981
982
983
984
985
986
Responsive DNN Adaptation for Video Analytics against Environment Shift via Hierarchical Mobile-Cloud Collaborations
987
988
989
990
991
992
993
994
995
996
997
998
999
1000
1001
1002
1003
1004
1005
1006
1007
1008
1009
1010
1011
1012
1013
1014
1015
1016
1017
1018
1019
1020
1021
1022
1023
1024
1025
1026
1027
1028
1029
1030
1031
1032
1033
1034
1035
1036
1037
1038
1039
1040
1041
1042
1043
10441 2 4 6 8
Device Number
0.2
0.3
0.4
Detection mAP
1 2 4 6 8
Device Number
0.60
0.65
0.70
0.75
0.80
Classification ACC.
1 2 4 6 8
Device Number
0.45
0.50
0.55
0.60
Segmentation MIoU
MOCHA RECL ODIN NO ADAPTATION Ekya
Figure 13: End-to-end evaluation of the recovery accu-
racy in object detection and image classification.1 2 4 6 8
Device Number
0
5
10
15
Response Delay (s)
0.47
1 2 4 6 8
Device Number
100
300
500
Retraining Time (s)
147
MOCHA RECL ODIN
Figure 14: Response delay and retraining time compari-
son. Object detection task is used.120 140 160 180
Retraining Time (s)
0.0
0.5
1.0
CDF
(a) 2 Mobile Devices
100 150 200 250 300
Retraining Time (s)
0.0
0.5
1.0
CDF
(b) 4 Mobile Devices
100 200 300 400
Retraining Time (s)
0.0
0.5
1.0
CDF
(c) 6 Mobile Devices
0 250 500 750
Retraining Time (s)
0.0
0.5
1.0
CDF
(d) 8 Mobile Devices
MOCHA RECL ODIN
Figure 15: CDF of retraining time across different numbers of devices.
During runtime, the encoder generates an embedding vector for
the input data, and ODIN selects the model corresponding to the
cluster whose centroid is closest to the embedding vector. In our
evaluation, we use the L2 distance as the similarity measure.
• Ekya: It enables retraining and inference to co-exist on the edge
device without model reuse. We utilize Ekya’s microprofiler and
thief scheduler to manage model retraining jobs for a fair com-
parision. Despite advanced resource-sharing mechanisms, Ekya
experiences out-of-band profiling overhead, which diminishes
overall responsiveness.
• RECL: It enables both retraining and reuse purely on the cloud.
We implemented RECL as described in their paper (model selec-
tor, safety checker, teacher labeler, and update modules released
in RECL). It maintains a gate network for initial model selection,
followed by a safety check with a validation dataset. Despite its
effective model reuse, RECL overlooks the network overhead
and focuses much on the update of the gate network.
7.2 End-to-end Evaluation
7.2.1 Recovery Accuracy. This is the end-to-end quality assess-
ment of all frameworks upon domain shifts. 12 domains are in-
cluded and 3 attributes of semantics are used. The recovery accu-
racy results of MOCHA and the baselines on all domain change
sequences are presented in Figure 13. MOCHA consistently outper-
forms all baselines under different numbers of connected mobile
devices, by up to 6.8% in the object detection task, up to 4.2% in the
image classification task and up to 3.8% in the semantic segmen-
tation task, due to its advanced hierarchical adaptation strategy,
allowing faster reuse and efficient fine-tuning.
7.2.2 Response Efficiency. We next compare the response de-
lay between different adaptation algorithms with model reuse in
Figure 14. MOCHA achieves the shortest response delay, 35.5×
shorter than the second-best approach. Moreover, MOCHA exhibits
better scalability in retraining time when more mobile devices are
connected to the cloud. In Figure 15, MOCHA demonstrates supe-
rior robustness in retraining time compared to baselines. It expe-
riences only a modest increase in retraining time as the number
of devices grows, resulting in a 1.34× increase. In contrast, RECL
shows a 4.03× increase due to the accumulation of ineffective re-
training tasks, and ODIN shows a 2.91× increase because of its
inefficiency in managing real-world data drift.
7.2.3 Adaptation Analysis. We use example traces to analyze
the adaptation collaborations in MOCHA. The same domain se-
quences are evaluated for all frameworks with object detection,
and 4 devices are connected to the cloud.
In the reuse process (Figure 16), upon a domain shift, MOCHA’s
on-device reuse quickly recovers the accuracy through onboard
model reuse, while both ODIN and RECL need to wait for the dis-
patched model from the cloud, creating delays in response. “Cache
Hit” and “Cache Miss” in MOCHA only differ in whether the ex-
pert model for the new domain is cached onboard. “MOCHA Cache
Hit” finishes with onboard model reuse, providing the best over-
all accuracy, while “MOCHA Cache Miss” partially resolves with
onboard cache and goes through the second reuse when the best
expert model is dispatched, which still surpasses RECL on the re-
covery accuracy. Although ODIN finishes the check and dispatch
quickly, it leads to suboptimal recovery accuracy due to the less
effective embedding manifold.
In Figure 17, we plot the inference accuracy starting from an
empty cloud model database, including MOCHA, ODIN, RECL, and
the Oracle framework that has sufficient cloud computing resources
and bandwidth for multiple retraining tasks. The system ingests 3
hours of video featuring 15 domains. MOCHA exhibits a rapid in-
crease in accuracy due to its superior semantic taxonomy and fine-
tuning mechanisms, whereas RECL shows slower improvement.
Both MOCHA and RECL can approach Oracle’s performance given
enough time to expand the model database, while ODIN falls short
for a less effective embedding manifold.
9
1045
1046
1047
1048
1049
1050
1051
1052
1053
1054
1055
1056
1057
1058
1059
1060
1061
1062
1063
1064
1065
1066
1067
1068
1069
1070
1071
1072
1073
1074
1075
1076
1077
1078
1079
1080
1081
1082
1083
1084
1085
1086
1087
1088
1089
1090
1091
1092
1093
1094
1095
1096
1097
1098
1099
1100
1101
1102
Anon.
1103
1104
1105
1106
1107
1108
1109
1110
1111
1112
1113
1114
1115
1116
1117
1118
1119
1120
1121
1122
1123
1124
1125
1126
1127
1128
1129
1130
1131
1132
1133
1134
1135
1136
1137
1138
1139
1140
1141
1142
1143
1144
1145
1146
1147
1148
1149
1150
1151
1152
1153
1154
1155
1156
1157
1158
1159
11600 5 10 15
Response Time (s)
0.2
0.4
0.6
0.8
mAP
MOCHA Cache Hit MOCHA Cache Miss RECL ODIN
Figure 16: Practical reuse example.0 1 2 3
Wall-clock Time (hours)
20
30
40
50
mAP
Oracle MOCHA RECL ODIN Figure 17: Practical adaptation example over time.2 4 8
Device Number
0.0
0.2
0.4
Detection mAP
2 4 8
Device Number
0.6
0.7
0.8
Classification ACC.
2 4 8
Device Number
0.4
0.5
0.6
Segmentation MIoU
MOCHA RECL NoFT NoRU
Figure 18: Impact of mobile fine-tuning and mobile selec-
tion. Both MOCHA and NoFT use the semantic taxonomy
for model selection while RECL uses a gate network. NoFT
lacks fine-tuning in MOCHA. NoRU has no model selection
or reuse.
7.3 Micro Experiemnts
7.3.1 Model selection and fine-tuning. In a model switch pro-
cess, the traditional approach involves mobile-cloud collaborative
model selection and model reuse with a gate network. In contrast,
MOCHA implements all model selection, reuse and fine-tuning at
the edge. Thus, it is not fair to directly compare MOCHA’s light-
weight semantic taxonomy with the gate network in model selec-
tion. To illustrate the contributions of each step within MOCHA,
we compare the performance of four methods: MOCHA, RECL,
NoFT(MOCHA without fine-tuning), and NoRU (Ekya without reuse).
Results are presented in Figure 18. It is evident that NoRU, utilizing
only lightweight model selection, does not have an accuracy advan-
tage over RECL (though it demonstrates significant improvements
in responsiveness and scalability). However, the incorporation of
reuse allows NoFT to achieve better performance than NoRU. Once
fine-tuning is included, MOCHA surpasses RECL in accuracy as
well. This is because we are willing to accept a less precise model
selection method than the gate network in exchange for respon-
siveness and lightweight performance while fine-tuning can en-
sure the accuracy of MOCHA.
7.3.2 OOD threshold performance. In Figure 19, we compare
the precision and recall under different �� of the boundary point
in domain shift detection (§4.1). When �� >= 0.4, the recall ex-
ceeds 0.95, which means it is inclusive in detecting potential do-
main shifts. With �� increases, the precision decreases to 0.1, which
means OOD triggers false positives without actual domain shifts.
Thus, “�� = 0.4” turns out to be the best configuration.
7.3.3 Adaptation ratio vs. Mobile device number As more
mobile devices are connected, the adaptation ratios for reuse, fine-
tuning, and retraining change, as illustrated in Figure 20. With
more devices, each device can leverage models in the model DB
trained from other devices. This boosts the probability of reuse
while reducing the need for fine-tuning and retraining, enhancing
the scalability of MOCHA.
Table 3: Mobile inference speed and overhead
Methods Speed
(ms/img)
Throughput
(FPS)
Memory
(GB)
Power
(W)
Inference Only 181 5.5 1.8 5.37
RECL 243 4.1 2.0 6.15
MOCHA no Adaptation 208 4.9 2.2 5.72
with Adaptation 354 2.8 4.8 10.96
7.4 Ablation Studies
7.4.1 Cloud Retraining Scheduler. When handling multiple re-
training tasks on the cloud, the scheduler performs better using a
“multi-level queue (MLQ)” algorithm compared to a simple First-In-
First-Out (FIFO) approach. We show the accuracy ratios (MLQ/FIFO)
in Figure 21. With an increasing number of devices, more retrain-
ing tasks are parallelized, and the scheduler can optimize task or-
dering, leading to a better overall performance by up to 1.23× in
object detection and 1.12× in image classification.
7.4.2 Mobile model cache. In Figure 22, we compare the MOCHA’s
accuracy with and without the mobile model cache in sequences
including frequent domain shifts. The sequences generate domain
shifts of existing domains in model DB with fixed numbers of win-
dows and we only launch reuse in MOCHA. Eliminating the model
cache, MOCHA experiences an accuracy drop of up to 11% and
13% respectively in two tasks. The average reuse time increases to
15.2s and is slightly influenced by the queuing delay on the cloud,
which makes MOCHA less competitive in responsiveness. It con-
firms that the device model cache is the key factor in optimizing
the responsiveness of MOCHA.
7.5 Mobile Overhead
We measure the inference performance and mobile overhead of
MOCHA, RECL, and the “Inference Only” baseline in Table 3. Com-
pared to RECL, during most non-domain-shifting periods without
adaptations (without Adap.), MOCHA consumes less power by 7%
and reaches faster speed by 19% due to the reduced need for fre-
quent data transfers, but extra memory by 10% because of detec-
tion. In potential shift time with no fine-tuning, MOCHA consumes
the same overhead as RECL, while its power consumption and
memory consumption increase by 2.4× and 1.78× respectively, and
its inference speed decreases 32% during the fine-tuning (with Adap.).
The resource overhead of MOCHA is generally within an accept-
able range.
8 Related Work
Video Analytics System. Video analytics systems aim to achieve
high inference accuracy while minimizing energy use and response
time through techniques like model distillation [6, 34, 36, 43], ar-
chitecture pruning [59, 60, 83, 85], configuration adaptation [29, 31,
10
1161
1162
1163
1164
1165
1166
1167
1168
1169
1170
1171
1172
1173
1174
1175
1176
1177
1178
1179
1180
1181
1182
1183
1184
1185
1186
1187
1188
1189
1190
1191
1192
1193
1194
1195
1196
1197
1198
1199
1200
1201
1202
1203
1204
1205
1206
1207
1208
1209
1210
1211
1212
1213
1214
1215
1216
1217
1218
Responsive DNN Adaptation for Video Analytics against Environment Shift via Hierarchical Mobile-Cloud Collaborations
1219
1220
1221
1222
1223
1224
1225
1226
1227
1228
1229
1230
1231
1232
1233
1234
1235
1236
1237
1238
1239
1240
1241
1242
1243
1244
1245
1246
1247
1248
1249
1250
1251
1252
1253
1254
1255
1256
1257
1258
1259
1260
1261
1262
1263
1264
1265
1266
1267
1268
1269
1270
1271
1272
1273
1274
1275
12760.3 0.4 0.5 0.6 0.7
k
0.0
0.5
1.0
Recall
0.3 0.4 0.5 0.6 0.7
k
0.0
0.2
0.4
Precision
Figure 19: OOD threshold performances by the hyper-
parameter ��.1 2 4 6 8
Device Number
0.00
0.25
0.50
0.75
1.00
Adaptation Ratio Reuse Fine-tuning Retraining Figure 20: Adaptation ratio changes across different
numbers of devices.2 4 6 8
Device Number
1.0
1.1
1.2
1.3
Detection Ratio
2 4 6 8
Device Number
1.0
1.1
1.2
Classification Ratio
2 4 6 8
Device Number
1.0
1.1
1.2
Segmentation Ratio
Figure 21: Cloud retraining scheduler comparison. Both
ratios represent the comparison of Multi-Level Queue
(MLQ) over First-In-First-Out (FIFO).1/8 1/6 1/4 1/2
Shift Frequency
0.25
0.50
0.75
Detection mAP
1/8 1/6 1/4 1/2
Shift Frequency
0.6
0.7
0.8
0.9
Classification ACC.
1/8 1/6 1/4 1/2
Shift Frequency
0.45
0.50
0.55
0.60
0.65
Segmentation MIoU
With Cache Without Cache
Figure 22: Impact of mobile model cache. Shift frequency
represents the reciprocal of the domain shift period, mea-
sured in the number of windows.
56, 91, 92], frame selection [12, 14, 45] and DNN feature reusing [22,
27, 30, 84]. The closest to MOCHA is model distillation, where
lightweight models are generated to perform on a specific video
scene [33, 34, 40]. It designs strategies to choose suitable experts
based on model retraining and model selection. Retraining tech-
niques train the lightweight models on the latest video frames [15,
36, 58] or on the most relevant images from the training set [66].
Selection techniques maintain and then select a model from a col-
lection of history models [74] or a cascade of models with increas-
ing capacities [8, 66]. Unlike traditional methods, MOCHA offloads
tasks to devices, improving responsiveness and scalability with an
on-device model cache and fine-tuning.
Model Selection under data drifts. Model selection in a collec-
tion of expert models has gained considerable attention, partic-
ularly in Mixture-of-Experts (MoE) and autoencoders (AE). Tra-
ditional MoE methods [37, 38, 64, 65, 69], which rely on a gate
network, reduce compute costs but necessitate enough memory
for loading models and frequent retraining for the gate network.
While AE techniques [1, 74, 80] project input data to a latent space
and map new models to a region in the latent space with limited
retraining but perform poorly facing domain shifts. In contrast,
MOCHA employs an FM and a semantics-based model taxonomy
for on-device selection, excelling in few-shot or zero-shot scenar-
ios with minimal updates (§2.2.2).
Continuous learning on the devices. In ML literature, CL for
mobile devices has been explored in notable works [23, 39] in trade-
offs between performance, storage, memory, and compute costs.
Recent studies [6, 54] highlight its benefits, motivating offloading
adaptations to leverage their natural high response advantages. In
MOCHA, on-device reuse and fine-tuning ensure responsiveness
and scalability, aligning with our research objectives.
9 Conclusion
With cloud offloading being the mainstream solution for contin-
uous mobile video analytics, this paper demonstrated that hierar-
chical model adaptation through mobile-cloud collaboration offers
significant potential in optimizing the responsiveness of adapta-
tion. We presented MOCHA, a mobile-cloud collaborative contin-
uous model adaptation framework, which organically integrates
efficient onboard model reuse and fine-tuning with backend model
retrieval and retraining on the cloud, achieving improved mobile
responsiveness and cloud scalability in our evaluations.
Still, our current work has limited optimization for replacement
strategies of the mobile model cache. And model management on
the cloud with numerous devices connected can be further devel-
oped to reduce memory overhead and adaptation delays. We hope
our findings can stimulate further research into harnessing the full
potential of the synergy between model reuse and model retrain-
ing in mobile video analytics systems.
11
1277
1278
1279
1280
1281
1282
1283
1284
1285
1286
1287
1288
1289
1290
1291
1292
1293
1294
1295
1296
1297
1298
1299
1300
1301
1302
1303
1304
1305
1306
1307
1308
1309
1310
1311
1312
1313
1314
1315
1316
1317
1318
1319
1320
1321
1322
1323
1324
1325
1326
1327
1328
1329
1330
1331
1332
1333
1334
Anon.
1335
1336
1337
1338
1339
1340
1341
1342
1343
1344
1345
1346
1347
1348
1349
1350
1351
1352
1353
1354
1355
1356
1357
1358
1359
1360
1361
1362
1363
1364
1365
1366
1367
1368
1369
1370
1371
1372
1373
1374
1375
1376
1377
1378
1379
1380
1381
1382
1383
1384
1385
1386
1387
1388
1389
1390
1391
1392
References
[1] R. Aljundi, P. Chakravarty, and T. Tuytelaars. Expert gate: Lifelong learning
with a network of experts. In Proceedings of the IEEE conference on computer
vision and pattern recognition, pages 3366–3375, 2017.
[2] K. Apicharttrisorn, J. Chen, V. Sekar, A. Rowe, and S. V. Krishnamurthy. Break-
ing edge shackles: Infrastructure-free collaborative mobile augmented reality.
In Proceedings of the 20th ACM Conference on Embedded Networked Sensor Sys-
tems, SenSys ’22, page 1–15, New York, NY, USA, 2023. Association for Comput-
ing Machinery.
[3] H. Bao, Z. Zhou, J. Xie, Q. Huang, F. Xu, and X. Chen. COUPLE: Accelerating
Video Analytics on Heterogeneous Mobile Processors. Association for Computing
Machinery, New York, NY, USA, 2023.
[4] R. Barjami, A. Miele, and L. Mottola. Intermittent inference: Trading a 1% accu-
racy loss for a 1.9x throughput speedup. In J. Liu, Y. Shu, J. Chen, Y. He, and
R. Tan, editors, Proceedings of the 22nd ACM Conference on Embedded Networked
Sensor Systems, SenSys 2024, Hangzhou, China, November 4-7, 2024, pages 647–
660. ACM, 2024.
[5] S. Beaulieu, L. Frati, T. Miconi, J. Lehman, K. O. Stanley, J. Clune, and N. Cheney.
Learning to continually learn. arXiv preprint arXiv:2002.09571, 2020.
[6] R. Bhardwaj, Z. Xia, G. Ananthanarayanan, J. Jiang, Y. Shu, N. Karianakis,
K. Hsieh, P. Bahl, and I. Stoica. Ekya: Continuous learning of video analyt-
ics models on edge compute servers. In 19th USENIX Symposium on Networked
Systems Design and Implementation (NSDI 22), pages 119–135, 2022.
[7] L. Butler, T. Yigitcanlar, and A. Paz. Smart urban mobility innovations: A com-
prehensive review and evaluation. Ieee Access, 8:196034–196049, 2020.
[8] J. Cao, R. Hadidi, J. Arulraj, and H. Kim. Thia: Accelerating video analyt-
ics using early inference and fine-grained query planning. arXiv preprint
arXiv:2102.08481, 2021.
[9] Q. Cao, H. Xue, T. Liu, X. Wang, H. Wang, X. Zhang, and L. Su. mmclip: Boosting
mmwave-based zero-shot har via signal-text alignment. In Proceedings of the
22nd ACM Conference on Embedded Networked Sensor Systems, SenSys ’24, page
184–197, New York, NY, USA, 2024. Association for Computing Machinery.
[10] L.-C. Chen, Y. Zhu, G. Papandreou, F. Schroff, and H. Adam. Encoder-decoder
with atrous separable convolution for semantic image segmentation. In Proceed-
ings of the European conference on computer vision (ECCV), pages 801–818, 2018.
[11] M. Chen, H. Chen, and S. Niu. Urinespec: A lightweight near-infrared spec-
troscopy system for metabolite detection in urine. In Proceedings of the 22nd
ACM Conference on Embedded Networked Sensor Systems, SenSys ’24, page 799–
810, New York, NY, USA, 2024. Association for Computing Machinery.
[12] T. Y.-H. Chen, L. Ravindranath, S. Deng, P. Bahl, and H. Balakrishnan. Glimpse:
Continuous, real-time object recognition on mobile devices. In Proceedings of
the 13th ACM conference on embedded networked sensor systems, pages 155–168,
2015.
[13] T. Contributors. Torchvision: Pytorch’s computer vision library, 2016–. Ac-
cessed: 2024-06-30.
[14] M. Dasari, K. Kahatapitiya, S. R. Das, A. Balasubramanian, and D. Samaras. Swift:
Adaptive video streaming with layered neural codecs. In 19th USENIX Sympo-
sium on Networked Systems Design and Implementation (NSDI 22), pages 103–118,
2022.
[15] Y. Deng, S. Yue, T. Wang, G. Wang, J. Ren, and Y. Zhang. Fedinc: An exemplar-
free continual federated learning framework with small labeled data. In Proceed-
ings of the 21st ACM Conference on Embedded Networked Sensor Systems, SenSys
’23, page 56–69, New York, NY, USA, 2024. Association for Computing Machin-
ery.
[16] J. A. Donenfeld and contributors. Wondershaper. https://github.com/magnific0/
wondershaper, 2002–2024. A script to limit bandwidth of a network interface.
[17] C. Fang, S. Liu, Z. Zhou, B. Guo, J. Tang, K. Ma, and Z. Yu. Adashadow: Respon-
sive test-time model adaptation in non-stationary mobile environments. arXiv
preprint arXiv:2410.08256, 2024.
[18] X. Fu, Y. Hu, P. Sutrave, P. A. Beerel, and B. Raghavan. Fireloc: Low-latency
multi-modal wildfire geolocation. In Proceedings of the 22nd ACM Conference
on Embedded Networked Sensor Systems, SenSys ’24, page 1–14, New York, NY,
USA, 2024. Association for Computing Machinery.
[19] M. Ghasemi, Z. Yang, M. Sun, H. Ye, Z. Xiong, J. Ghaderi, Z. Kostic, and G. Zuss-
man. Video-based social distancing evaluation in the cosmos testbed pilot site.
In Proceedings of the 27th Annual International Conference on Mobile Computing
and Networking, MobiCom ’21, page 874–876, New York, NY, USA, 2022. Asso-
ciation for Computing Machinery.
[20] S. Gui, H. Wang, H. Yang, C. Yu, Z. Wang, and J. Liu. Model compression with
adversarial robustness: A unified optimization framework. Advances in Neural
Information Processing Systems, 32, 2019.
[21] D. L. Guidoni, G. Maia, F. S. Souza, L. A. Villas, and A. A. Loureiro. Vehicular
traffic management based on traffic engineering for vehicular ad hoc networks.
IEEE Access, 8:45167–45183, 2020.
[22] P. Guo, B. Hu, and W. Hu. Mistify: Automating {DNN} model porting for {On-
Device} inference at the edge. In 18th USENIX Symposium on Networked Systems
Design and Implementation (NSDI 21), pages 705–719, 2021.
[23] T. L. Hayes and C. Kanan. Online continual learning for embedded devices.
arXiv preprint arXiv:2203.10681, 2022.
[24] K. He, X. Zhang, S. Ren, and J. Sun. Deep residual learning for image recognition.
In Proceedings of the IEEE conference on computer vision and pattern recognition,
pages 770–778, 2016.
[25] Y. He, C. Bian, J. Xia, S. Shi, Z. Yan, Q. Song, and G. Xing. Vi-map: Infrastructure-
assisted real-time hd mapping for autonomous driving. In Proceedings of the 29th
Annual International Conference on Mobile Computing and Networking, ACM Mo-
biCom ’23, New York, NY, USA, 2023. Association for Computing Machinery.
[26] Y. He, L. Ma, J. Cui, Z. Yan, G. Xing, S. Wang, Q. Hu, and C. Pan. Automatch:
Leveraging traffic camera to improve perception and localization of autonomous
vehicles. In Proceedings of the 20th ACM Conference on Embedded Networked
Sensor Systems, SenSys ’22, page 16–30, New York, NY, USA, 2023. Association
for Computing Machinery.
[27] K. Hsieh, G. Ananthanarayanan, P. Bodik, S. Venkataraman, P. Bahl, M. Phili-
pose, P. B. Gibbons, and O. Mutlu. Focus: Querying large video datasets with
low latency and low cost. In 13th USENIX Symposium on Operating Systems
Design and Implementation (OSDI 18), pages 269–286, 2018.
[28] I. K. Jain, S. M. M, and D. Bharadia. Commrad: Context-aware sensing-driven
millimeter-wave networks. In J. Liu, Y. Shu, J. Chen, Y. He, and R. Tan, editors,
Proceedings of the 22nd ACM Conference on Embedded Networked Sensor Systems,
SenSys 2024, Hangzhou, China, November 4-7, 2024, pages 633–646. ACM, 2024.
[29] S. Jain, G. Ananthanarayanan, J. Jiang, Y. Shu, and J. Gonzalez. Scaling video
analytics systems to large camera deployments. In Proceedings of the 20th Inter-
national Workshop on Mobile Computing Systems and Applications, pages 9–14,
2019.
[30] A. H. Jiang, D. L.-K. Wong, C. Canel, L. Tang, I. Misra, M. Kaminsky, M. A.
Kozuch, P. Pillai, D. G. Andersen, and G. R. Ganger. Mainstream: Dynamic
{Stem-Sharing} for {Multi-Tenant} video processing. In 2018 USENIX Annual
Technical Conference (USENIX ATC 18), pages 29–42, 2018.
[31] J. Jiang, G. Ananthanarayanan, P. Bodik, S. Sen, and I. Stoica. Chameleon: scal-
able adaptation of video analytics. In Proceedings of the 2018 conference of the
ACM special interest group on data communication, pages 253–266, 2018.
[32] G. Jocher, A. Stoken, J. Borovec, A. Chaurasia, L. Changyu, A. Hogan, J. Hajek,
L. Diaconu, Y. Kwon, Y. Defretin, et al. ultralytics/yolov5: v5. 0-yolov5-p6 1280
models, aws, supervise. ly and youtube integrations. Zenodo, 2021.
[33] D. Kang, P. Bailis, and M. Zaharia. Blazeit: Optimizing declarative aggrega-
tion and limit queries for neural network-based video analytics. arXiv preprint
arXiv:1805.01046, 2018.
[34] D. Kang, J. Emmons, F. Abuzaid, P. Bailis, and M. Zaharia. Noscope: optimizing
neural network queries over video at scale. arXiv preprint arXiv:1703.02529, 2017.
[35] M. Khani, G. Ananthanarayanan, K. Hsieh, J. Jiang, R. Netravali, Y. Shu, M. Al-
izadeh, and V. Bahl. {RECL}: Responsive {Resource-Efficient} continuous
learning for video analytics. In 20th USENIX Symposium on Networked Systems
Design and Implementation (NSDI 23), pages 917–932, 2023.
[36] M. Khani, P. Hamadanian, A. Nasr-Esfahany, and M. Alizadeh. Real-time video
inference on edge devices via adaptive model streaming. In Proceedings of the
IEEE/CVF International Conference on Computer Vision, pages 4572–4582, 2021.
[37] J. Z. Kolter and M. A. Maloof. Using additive expert ensembles to cope with
concept drift. In Proceedings of the 22nd international conference on Machine
learning, pages 449–456, 2005.
[38] J. Z. Kolter and M. A. Maloof. Dynamic weighted majority: An ensemble method
for drifting concepts. The Journal of Machine Learning Research, 8:2755–2790,
2007.
[39] Y. D. Kwon, J. Chauhan, A. Kumar, P. H. HKUST, and C. Mascolo. Exploring
system performance of continual learning for mobile and embedded sensing
applications. In 2021 IEEE/ACM Symposium on Edge Computing (SEC), pages
319–332. IEEE, 2021.
[40] J. Lee, P. Wang, R. Xu, V. Dasari, N. Weston, Y. Li, S. Bagchi, and S. Chaterji.
Benchmarking video object detection systems on embedded devices under re-
source contention. In Proceedings of the 5th International Workshop on Embedded
and Mobile Deep Learning, pages 19–24, 2021.
[41] K. Lee, K. Lee, H. Lee, and J. Shin. A simple unified framework for detecting out-
of-distribution samples and adversarial attacks. Advances in neural information
processing systems, 31, 2018.
[42] A. Li, J. Sun, X. Zeng, M. Zhang, H. Li, and Y. Chen. Fedmask: Joint computation
and communication-efficient personalized federated learning via heterogeneous
masking. In Proceedings of the 19th ACM Conference on Embedded Networked
Sensor Systems, SenSys ’21, page 42–55, New York, NY, USA, 2021. Association
for Computing Machinery.
[43] X. Li, Y. Li, Y. Li, T. Cao, and Y. Liu. Flexnn: Efficient and adaptive DNN infer-
ence on memory-constrained edge devices. In W. Shi, D. Ganesan, and N. D.
Lane, editors, Proceedings of the 30th Annual International Conference on Mobile
Computing and Networking, ACM MobiCom 2024, Washington D.C., DC, USA, No-
vember 18-22, 2024, pages 709–723. ACM, 2024.
[44] Y. Li, L. Liu, H. Li, W. Liu, Y. Chen, W. Zhao, J. Wu, Q. Wu, J. Liu, and Z. Lai. Stable
hierarchical routing for operational LEO networks. In W. Shi, D. Ganesan, and
N. D. Lane, editors, Proceedings of the 30th Annual International Conference on
12
1393
1394
1395
1396
1397
1398
1399
1400
1401
1402
1403
1404
1405
1406
1407
1408
1409
1410
1411
1412
1413
1414
1415
1416
1417
1418
1419
1420
1421
1422
1423
1424
1425
1426
1427
1428
1429
1430
1431
1432
1433
1434
1435
1436
1437
1438
1439
1440
1441
1442
1443
1444
1445
1446
1447
1448
1449
1450
Responsive DNN Adaptation for Video Analytics against Environment Shift via Hierarchical Mobile-Cloud Collaborations
1451
1452
1453
1454
1455
1456
1457
1458
1459
1460
1461
1462
1463
1464
1465
1466
1467
1468
1469
1470
1471
1472
1473
1474
1475
1476
1477
1478
1479
1480
1481
1482
1483
1484
1485
1486
1487
1488
1489
1490
1491
1492
1493
1494
1495
1496
1497
1498
1499
1500
1501
1502
1503
1504
1505
1506
1507
1508
Mobile Computing and Networking, ACM MobiCom 2024, Washington D.C., DC,
USA, November 18-22, 2024, pages 296–311. ACM, 2024.
[45] Y. Li, A. Padmanabhan, P. Zhao, Y. Wang, G. H. Xu, and R. Netravali. Reducto:
On-camera filtering for resource-efficient real-time video analytics. In Proceed-
ings of the Annual conference of the ACM Special Interest Group on Data Commu-
nication on the applications, technologies, architectures, and protocols for computer
communication, pages 359–376, 2020.
[46] C. Lin, Z. Zhang, H. Li, and J. Liu. Ecsrl: A learning-based scheduling framework
for ai workloads in heterogeneous edge-cloud systems. In Proceedings of the 19th
ACM Conference on Embedded Networked Sensor Systems, SenSys ’21, page 386–
387, New York, NY, USA, 2021. Association for Computing Machinery.
[47] N. Ling, X. Huang, Z. Zhao, N. Guan, Z. Yan, and G. Xing. Blastnet: Exploiting
duo-blocks for cross-processor real-time dnn inference. In Proceedings of the
20th ACM Conference on Embedded Networked Sensor Systems, SenSys ’22, page
91–105, New York, NY, USA, 2023. Association for Computing Machinery.
[48] H. Liu, C. Li, Q. Wu, and Y. J. Lee. Visual instruction tuning. In NeurIPS, 2023.
[49] J. Lu, A. Liu, F. Dong, F. Gu, J. Gama, and G. Zhang. Learning under concept drift:
A review. IEEE transactions on knowledge and data engineering, 31(12):2346–2363,
2018.
[50] Y. Lu, D. Ding, H. Pan, Y. Fu, L. Zhang, F. Tan, R. Wang, Y. Chen, G. Xue, and
J. Ren. M3cam: Extreme super-resolution via multi-modal optical flow for mo-
bile cameras. In J. Liu, Y. Shu, J. Chen, Y. He, and R. Tan, editors, Proceedings of
the 22nd ACM Conference on Embedded Networked Sensor Systems, SenSys 2024,
Hangzhou, China, November 4-7, 2024, pages 744–756. ACM, 2024.
[51] P. Luo, J. Hou, M. Yuan, G. Wu, Y. Yao, and X. Li. F2zip: Finetuning-free model
compression for scenario-adaptive embedded vision. In J. Liu, Y. Shu, J. Chen,
Y. He, and R. Tan, editors, Proceedings of the 22nd ACM Conference on Embedded
Networked Sensor Systems, SenSys 2024, Hangzhou, China, November 4-7, 2024,
pages 15–27. ACM, 2024.
[52] G. Lv, Q. Wu, Y. Liu, Z. Li, Q. Tan, F. Yang, W. Chen, Y. Ma, H. Guo, Y. Chen, and
G. Xie. Chorus: Coordinating mobile multipath scheduling and adaptive video
streaming. In Proceedings of the 30th Annual International Conference on Mobile
Computing and Networking, ACM MobiCom ’24, page 246–262, New York, NY,
USA, 2024. Association for Computing Machinery.
[53] G. Lv, Q. Wu, Y. Liu, Z. Li, Q. Tan, F. Yang, W. Chen, Y. Ma, H. Guo, Y. Chen,
and G. Xie. Chorus: Coordinating mobile multipath scheduling and adaptive
video streaming. In W. Shi, D. Ganesan, and N. D. Lane, editors, Proceedings of
the 30th Annual International Conference on Mobile Computing and Networking,
ACM MobiCom 2024, Washington D.C., DC, USA, November 18-22, 2024, pages
246–262. ACM, 2024.
[54] X. Ma, S. Jeong, M. Zhang, D. Wang, J. Choi, and M. Jeon. Cost-effective on-
device continual learning over memory hierarchy with miro. In Proceedings of
the 29th Annual International Conference on Mobile Computing and Networking,
pages 1–15, 2023.
[55] Z. Mahrez, E. Sabir, E. Badidi, W. Saad, and M. Sadik. Smart urban mobility:
When mobility systems meet smart data. IEEE Transactions on Intelligent Trans-
portation Systems, 23(7):6222–6239, 2021.
[56] Z. Meng, T. Wang, Y. Shen, B. Wang, M. Xu, R. Han, H. Liu, V. Arun, H. Hu,
and X. Wei. Enabling high quality {Real-Time} communications with adaptive
{Frame-Rate}. In 20th USENIX Symposium on Networked Systems Design and
Implementation (NSDI 23), pages 1429–1450, 2023.
[57] P. Molchanov, S. Tyree, T. Karras, T. Aila, and J. Kautz. Pruning convolutional
neural networks for resource efficient inference. arXiv preprint arXiv:1611.06440,
2016.
[58] R. T. Mullapudi, S. Chen, K. Zhang, D. Ramanan, and K. Fatahalian. Online
model distillation for efficient video inference. In Proceedings of the IEEE/CVF
International conference on computer vision, pages 3573–3582, 2019.
[59] A. Padmanabhan, N. Agarwal, A. Iyer, G. Ananthanarayanan, Y. Shu, N. Kar-
ianakis, G. H. Xu, and R. Netravali. Gemel: Model merging for {Memory-
Efficient},{Real-Time} video analytics at the edge. In 20th USENIX Sympo-
sium on Networked Systems Design and Implementation (NSDI 23), pages 973–994,
2023.
[60] T. Pan, K. Liu, X. Wei, Y. Qiao, J. Hu, Z. Li, J. Liang, T. Cheng, W. Su, J. Lu,
et al. {LuoShen}: A {Hyper-Converged} programmable gateway for {Multi-
Tenant} {Multi-Service} edge clouds. In 21st USENIX Symposium on Networked
Systems Design and Implementation (NSDI 24), pages 877–892, 2024.
[61] V. Panchenko, A. Zamula, S. Kavun, and I. Mikheev. Intelligent management of
the enterprise personnel security system. In 2018 IEEE 9th International Confer-
ence on Dependable Systems, Services and Technologies (DESSERT), pages 469–474.
IEEE, 2018.
[62] G. I. Parisi, R. Kemker, J. L. Part, C. Kanan, and S. Wermter. Continual lifelong
learning with neural networks: A review. Neural networks, 113:54–71, 2019.
[63] A. Paszke, S. Gross, F. Massa, A. Lerer, J. Bradbury, G. Chanan, T. Killeen, Z. Lin,
N. Gimelshein, L. Antiga, A. Desmaison, A. Kopf, E. Yang, Z. DeVito, M. Raison,
A. Tejani, S. Chilamkurthy, B. Steiner, L. Fang, J. Bai, and S. Chintala. Pytorch:
An imperative style, high-performance deep learning library. In Proceedings
of the 33rd International Conference on Neural Information Processing Systems,
pages 8024–8035. Curran Associates, Inc., 2019.
[64] C. Riquelme, J. Puigcerver, B. Mustafa, M. Neumann, R. Jenatton, A. Su-
sano Pinto, D. Keysers, and N. Houlsby. Scaling vision with sparse mixture
of experts. Advances in Neural Information Processing Systems, 34:8583–8595,
2021.
[65] N. Shazeer, A. Mirhoseini, K. Maziarz, A. Davis, Q. Le, G. Hinton, and J. Dean.
Outrageously large neural networks: The sparsely-gated mixture-of-experts
layer. arXiv preprint arXiv:1701.06538, 2017.
[66] H. Shen, S. Han, M. Philipose, and A. Krishnamurthy. Fast video classification
via adaptive cascading of deep models. In Proceedings of the IEEE conference on
computer vision and pattern recognition, pages 3646–3654, 2017.
[67] S. Shi, J. Cui, Z. Jiang, Z. Yan, G. Xing, J. Niu, and Z. Ouyang. Vips: real-time per-
ception fusion for infrastructure-assisted autonomous driving. In Proceedings of
the 28th Annual International Conference on Mobile Computing And Networking,
MobiCom ’22, page 133–146, New York, NY, USA, 2022. Association for Com-
puting Machinery.
[68] S. Shi, N. Ling, Z. Jiang, X. Huang, Y. He, X. Zhao, B. Yang, C. Bian, J. Xia, Z. Yan,
R. W. Yeung, and G. Xing. Soar: Design and deployment of A smart roadside
infrastructure system for autonomous driving. In W. Shi, D. Ganesan, and N. D.
Lane, editors, Proceedings of the 30th Annual International Conference on Mobile
Computing and Networking, ACM MobiCom 2024, Washington D.C., DC, USA, No-
vember 18-22, 2024, pages 139–154. ACM, 2024.
[69] Y. Shi, B. Paige, P. Torr, et al. Variational mixture-of-experts autoencoders for
multi-modal deep generative models. Advances in neural information processing
systems, 32, 2019.
[70] V. Sivaraman, P. Karimi, V. Venkatapathy, M. Khani, S. Fouladi, M. Alizadeh,
F. Durand, and V. Sze. Gemino: Practical and robust neural compression for
video conferencing. In 21st USENIX Symposium on Networked Systems De-
sign and Implementation (NSDI 24), pages 569–590, Santa Clara, CA, Apr. 2024.
USENIX Association.
[71] T. Srivastava, P. Khanna, S. Pan, P. Nguyen, and S. Jain. Unvoiced: Designing
an llm-assisted unvoiced user interface using earables. In J. Liu, Y. Shu, J. Chen,
Y. He, and R. Tan, editors, Proceedings of the 22nd ACM Conference on Embedded
Networked Sensor Systems, SenSys 2024, Hangzhou, China, November 4-7, 2024,
pages 784–798. ACM, 2024.
[72] B. Sudharsan, D. Sheth, S. Arya, F. Rollo, P. Yadav, P. Patel, J. G. Breslin, and
M. I. Ali. Elasticl: Elastic quantization for communication efficient collabora-
tive learning in iot. In Proceedings of the 19th ACM Conference on Embedded
Networked Sensor Systems, SenSys ’21, page 382–383, New York, NY, USA, 2021.
Association for Computing Machinery.
[73] J. Sun, A. Li, L. Duan, S. Alam, X. Deng, X. Guo, H. Wang, M. Gorlatova,
M. Zhang, H. Li, and Y. Chen. Fedsea: A semi-asynchronous federated learn-
ing framework for extremely heterogeneous devices. In Proceedings of the 20th
ACM Conference on Embedded Networked Sensor Systems, SenSys ’22, page 106–
119, New York, NY, USA, 2023. Association for Computing Machinery.
[74] A. Suprem, J. Arulraj, C. Pu, and J. Ferreira. Odin: Automated drift detection
and recovery in video analytics. Proceedings of the VLDB Endowment, 13(11).
[75] M. Tang, P. Teckchandani, J. He, H. Guo, and E. Soltanaghai. BSENSE: in-vehicle
child detection and vital sign monitoring with a single mmwave radar and syn-
thetic reflectors. In J. Liu, Y. Shu, J. Chen, Y. He, and R. Tan, editors, Proceedings
of the 22nd ACM Conference on Embedded Networked Sensor Systems, SenSys 2024,
Hangzhou, China, November 4-7, 2024, pages 478–492. ACM, 2024.
[76] P. Tong, M. Li, M. Li, J. Huang, and X. Hua. Large-scale vehicle trajectory re-
construction with camera sensing network. In Proceedings of the 27th Annual
International Conference on Mobile Computing and Networking, MobiCom ’21,
page 188–200, New York, NY, USA, 2021. Association for Computing Machin-
ery.
[77] J. Wang, J. Liu, and N. Kato. Networking and communications in autonomous
driving: A survey. IEEE Communications Surveys & Tutorials, 21(2):1243–1274,
2018.
[78] L. Wang, S. Jajodia, A. Singhal, A. Singhal, and X. Ou. Security risk analysis of
enterprise networks using probabilistic attack graphs. Springer, 2017.
[79] S. Wang, S. Yang, H. Li, X. Zhang, C. Zhou, C. Xu, F. Qian, N. Wang, and Z. Xu.
Pyramidfl: A fine-grained client selection framework for effiicient federated
learning. In 28th ACM Annual International Conference on Mobile Computing
and Networking, MobiCom 2022, pages 542–555. Association for Computing Ma-
chinery, 2022.
[80] T. Wang, J. Li, R. Wang, D. Kara, S. Liu, D. Wertheimer, A. Viros i Martin, R. Ganti,
M. Srivatsa, and T. Abdelzaher. Sudokusens: Enhancing deep learning robust-
ness for iot sensing applications using a generative approach. In Proceedings
of the 21st ACM Conference on Embedded Networked Sensor Systems, SenSys ’23,
page 15–27, New York, NY, USA, 2024. Association for Computing Machinery.
[81] M. Wong, M. Ramanujam, G. Balakrishnan, and R. Netravali. MadEye: Boost-
ing live video analytics accuracy with adaptive camera configurations. In 21st
USENIX Symposium on Networked Systems Design and Implementation (NSDI 24),
pages 549–568, Santa Clara, CA, Apr. 2024. USENIX Association.
[82] M. Woźniak, M. Wieczorek, and J. Siłka. Deep neural network with transfer
learning in remote object detection from drone. In Proceedings of the 5th inter-
national ACM Mobicom workshop on drone assisted wireless communications for
13
1509
1510
1511
1512
1513
1514
1515
1516
1517
1518
1519
1520
1521
1522
1523
1524
1525
1526
1527
1528
1529
1530
1531
1532
1533
1534
1535
1536
1537
1538
1539
1540
1541
1542
1543
1544
1545
1546
1547
1548
1549
1550
1551
1552
1553
1554
1555
1556
1557
1558
1559
1560
1561
1562
1563
1564
1565
1566
Anon.
1567
1568
1569
1570
1571
1572
1573
1574
1575
1576
1577
1578
1579
1580
1581
1582
1583
1584
1585
1586
1587
1588
1589
1590
1591
1592
1593
1594
1595
1596
1597
1598
1599
1600
1601
1602
1603
1604
1605
1606
1607
1608
1609
1610
1611
1612
1613
1614
1615
1616
1617
1618
1619
1620
1621
1622
1623
1624
5G and beyond, pages 121–126, 2022.
[83] B. Wu, X. Dai, P. Zhang, Y. Wang, F. Sun, Y. Wu, Y. Tian, P. Vajda, Y. Jia, and
K. Keutzer. Fbnet: Hardware-aware efficient convnet design via differentiable
neural architecture search. In Proceedings of the IEEE/CVF conference on com-
puter vision and pattern recognition, pages 10734–10742, 2019.
[84] M. Xu, M. Zhu, Y. Liu, F. X. Lin, and X. Liu. Deepcache: Principled cache for
mobile deep vision. In Proceedings of the 24th annual international conference on
mobile computing and networking, pages 129–144, 2018.
[85] R. Xu, R. Kumar, P. Wang, P. Bai, G. Meghanath, S. Chaterji, S. Mitra, and
S. Bagchi. Approxnet: Content and contention-aware video object classifica-
tion system for embedded clients. ACM Transactions on Sensor Networks (TOSN),
18(1):1–27, 2021.
[86] Z. Xue, Y. Song, Z. Mi, L. Chen, Y. Xia, and H. Chen. Powerinfer-2: Fast large
language model inference on a smartphone. arXiv preprint arXiv:2406.06282,
2024.
[87] S. Ye, L. Zeng, X. Chu, G. Xing, and X. Chen. Asteroid: Resource-efficient hy-
brid pipeline parallelism for collaborative dnn training on heterogeneous edge
devices. In Proceedings of the 30th Annual International Conference on Mobile
Computing and Networking, ACM MobiCom ’24, page 312–326, New York, NY,
USA, 2024. Association for Computing Machinery.
[88] F. Yu, H. Chen, X. Wang, W. Xian, Y. Chen, F. Liu, V. Madhavan, and T. Darrell.
Bdd100k: A diverse driving dataset for heterogeneous multitask learning. In
IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR), June
2020.
[89] E. Yurtsever, J. Lambert, A. Carballo, and K. Takeda. A survey of autonomous
driving: Common practices and emerging technologies. IEEE access, 8:58443–
58469, 2020.
[90] X. Zeng, B. Fang, H. Shen, and M. Zhang. Distream: scaling live video analytics
with workload-adaptive distributed edge intelligence. In Proceedings of the 18th
Conference on Embedded Networked Sensor Systems, SenSys ’20, page 409–421,
New York, NY, USA, 2020. Association for Computing Machinery.
[91] B. Zhang, X. Jin, S. Ratnasamy, J. Wawrzynek, and E. A. Lee. Awstream: Adaptive
wide-area streaming analytics. In Proceedings of the 2018 Conference of the ACM
Special Interest Group on Data Communication, pages 236–252, 2018.
[92] H. Zhang, G. Ananthanarayanan, P. Bodik, M. Philipose, P. Bahl, and M. J. Freed-
man. Live video analytics at scale with approximation and {Delay-Tolerance}.
In 14th USENIX Symposium on Networked Systems Design and Implementation
(NSDI 17), pages 377–392, 2017.
[93] Y. Zhang, T. Gu, and X. Zhang. Mdldroidlite: a release-and-inhibit control ap-
proach to resource-efficient deep neural networks on mobile devices. In Proceed-
ings of the 18th Conference on Embedded Networked Sensor Systems, SenSys ’20,
page 463–475, New York, NY, USA, 2020. Association for Computing Machinery.
[94] Z. Zhao, N. Ling, N. Guan, and G. Xing. Miriam: Exploiting elastic kernels for
real-time multi-dnn inference on edge gpu. In Proceedings of the 21st ACM Con-
ference on Embedded Networked Sensor Systems, SenSys ’23, page 97–110, New
York, NY, USA, 2024. Association for Computing Machinery.
[95] J. Zheng, Z. Li, F. Qian, W. Liu, H. Lin, Y. Liu, T. Xu, N. Zhang, J. Wang, and
C. Zhang. Rethinking process management for interactive mobile systems. In
W. Shi, D. Ganesan, and N. D. Lane, editors, Proceedings of the 30th Annual Inter-
national Conference on Mobile Computing and Networking, ACM MobiCom 2024,
Washington D.C., DC, USA, November 18-22, 2024, pages 215–229. ACM, 2024.
14

==> text/discussion.tex <==
\section{Limitations and Discussion} \label{sec:discussion}
In this section, we briefly discuss the existing limitations in our systems. Some lessons, experiences, and future work are also included.


